Mobile Network Slicing under Demand Uncertainty: A Stochastic Programming Approach

Network slicing enables the deployment of multiple dedicated virtual sub-networks, i.e. slices on a shared physical infrastructure. Unlike traditional one-size-fits-all resource provisioning schemes, each network slice (NS) in 5G is tailored to the specific service requirements of a group of customers. An end-to-end (E2E) mobile NS orchestration requires the simultaneous provisioning of computing, storage, and networking resources across the core network (CN) and the radio access network (RAN). Constant temporospatial changes in mobile user demand profiles further complicate the E2E NSs resource provisioning beyond the limits of the existing best-effort schemes that are only effective under accurate demand forecasts for all slices. This paper proposes a practical two-time-scale resource provisioning framework for E2E network slicing under demand uncertainty. At each macro-scale instance, we assume that only the spatial probability distribution of the NS demands is available. We formulate the NSs resource allocation problem as a stochastic mixed integer program (SMIP) with the objective of minimizing the total resource cost at the CN and the RAN. At each microscale instance, utilizing the exact slice demand profiles, a linear program is solved to jointly minimize the unsupported traffic and the resource cost at the RAN. We verify the effectiveness of our resource allocation scheme through numerical experiments.

==> IEEE NetSoft 2023 (1)/Introduction.tex <==
\section{Introduction}
Softwarization based on network function virtualization (NFV) and software-defined networking (SDN) is envisioned to realize programmable control and management of network resources in next-generation mobile networks \cite{barakabitze20205g}. Building upon SDN and NFV as the enabling technologies, \emph{network slicing} allows the physical infrastructure to be segmented into several logically-isolated sub-networks each customized to the specific quality of service (QoS) requirements of an application. Such a dedicated resource provisioning framework results in significant reductions in network management and equipment costs \cite{wireless-virtu}. 


In the paradigm of 5G enhanced by \emph{network slicing}, mobile network operators (MNOs) manage and set up network slices (NSs) and provide service providers (SPs) with an on-demand scalable delivery of network services \cite{5g-NS}. The SPs, a.k.a. \textit{tenants}, dedicate NSs to customers with various QoS requirements in a sustainable manner. A mobile NS spans across multiple domains, namely the radio access network (RAN), the core network (CN), and the transport network (TN), forming an end-to-end (E2E) sub-network. 

In contrast to the traditional static allocation of resources \cite{RL-NS}, 5G RAN slicing introduces the capability of sharing physical network infrastructure among mobile virtual network operators (MVNOs). Consequently, the radio resources such as time, frequency, and power are reserved on the fly based on dynamic user demands. Each sub-slice corresponding to a specific part of the network includes service function chains (SFCs) consisting of multiple virtual network functions (VNFs) and physical network functions (PNFs). Designing E2E NSs requires resource provisioning across heterogeneous physical and virtual network infrastructures each having specific technical constraints. On the other hand, with a proliferation of advanced and diverse digital services such as hologram video streaming and multi-sensory extended reality, the sixth-generation mobile system (6G) is envisioned to facilitate massive and extremely heterogeneous \emph{network slicing} where tenancy would be extended further to the end user \cite{6G-slice}. 
% Following the anything-as-a-Service (XaaS) paradigm \cite{XaaS}, the concept of network slice as a Service (NSaaS) has been introduced  to provide customized E2E slice by horizontally splitting computation and communication resources. 
In such architectures with slicing-aware user equipment (UE), new challenges are introduced. For instance, UE mobility should be considered by the SPs as part of the slice setup and management procedure \cite{ns-scal-flex}. 


Although \emph{network slicing} promises to enhance the agility of next-generation mobile networks, practical NS deployment faces key challenges among which the uncertainty in the demand for different slices stands out. In practice, the shared physical network resources must be dynamically and efficiently allocated to logical NSs based on changing user demands. However, the existing resource provisioning methods for \emph{network slicing} are typically performed in a best-effort manner \cite{su2019resource}. Consequently, there is no guarantee that resources allocated to different slices will be sufficient to support constantly-varying demand profiles. Besides the dynamicity of the user demand profiles, the variation in the infrastructure resource availability status may degrade the slice QoS compared to the service level agreement (SLA) promised by the SPs \cite{luu2021uncertainty}. \emph{Elasticity} which refers to the availability of resources in an adaptive way according to user demands plays a critical role in meeting the differentiated QoS requirements of different slices while avoiding resource under-utilization or over-utilization \cite{khan2020network}. 

In this paper, we propose a novel approach to optimize the E2E resource provisioning for \emph{network slicing} under demand uncertainty. Stochastic programming is a powerful tool to address optimization under uncertainty. We consider the joint resource allocation of next-generation RAN (NG-RAN) and 5G core (5GC) for different slices as shown in Fig. \ref{fig:E2ENS}. 
% We propose a two-timescale solution that handles the resource optimization of NG-RAN and 5GC adaptively in a hierarchical manner.
In our proposed solution, the RAN slicing is triggered more frequently (i.e. has a shorter life cycle) compared to the CN segment, due to the existence of more dynamic parameters in the wireless network such as user mobility and channel conditions. Therefore, our algorithm operates at two time scales. At each macro-scale instance, we assume that only the spatial probability distribution of the network slice demands is available. We formulate the network slices resource allocation problem as a stochastic mixed integer program (SMIP) with the objective of minimizing the total resource cost at the CN and the RAN. At each micro-scale instance,  utilizing the exact slice demand profiles, a linear program is solved to jointly minimize the unsupported traffic and the resource provisioning cost at the RAN.


% At each decision time instance, we assume that the probability distribution of the objective of the problem is to minimize the total provisioning cost while satisfying the infrastructure capacity constraints and the QoS requirements of each slice. 

The remainder of the paper is organized as follows. In section~\ref{sec:related}, we present the literature review.  Section~\ref{sec:sys} describes the system model. The problem formulation is provided in section~\ref{sec:formulation_thesis}. The proposed solution is presented in section~\ref{sec:solution}, while the numerical results are provided in section \ref{sec:evaluation}. Finally, we highlight our conclusions in section \ref{sec:conclusion}.

% \section{Summary of Contribution}
% \label{sec:contribution}
% The main contribution of this paper is as follows:
% \begin{itemize}
%     \item We propose a novel method to formulate the resource provisioning problem of E2E network slicing under demand uncertainty using two-stage stochastic programming.
%     \item Our proposed framework is robust against unknown network slice demands by incorporating uncertainties for different network slices.
%     \item In order to tackle the time complexity of the proposed method due to integer variables, we consider two approximation methods and show their efficacy through extensive simulations.
% \end{itemize}

% Based on network slicing, each tenant The ever increasing volume of traffic demand and new bandwidth-hungry mobile services degrade the performance of the present mobile networks. Moreover, the users' traffic patterns are becoming more diverse and dynamic as a result of the creation of new services with different quality of service (QoS) requirements such as data rate and latency. In order to cope with this new paradigm, software defined networking (SDN) and network function virtualization (NFV) are proposed. Building on SDN and NFV technologies as enablers, network slicing is envisioned as on of the key enablers of 5G systems, allowing the physical infrastructure to be segmented into a number of logically isolated sub-networks each instantiated for a network service with specific QoS requirements. From business model perspective, network slicing introduces new capabilities such as allowing telecommmunication operators to lease a virtualized slice of their infrastructure to tenants such as automotive, e-health, factories, vehicular networks, IoT, etc., multiplexed over a single physical infrastructure. Therefore, efficient Network Slicing is vital to provide flexible and dynamic virtual networks and serve spatiotemporal traffic patterns. 

% A Network Slice (NS), in the context of 5G, is composed of sub-slices covering the Radio Access Network (RAN), Core Network (CN) and the transport network. Each sub-slice is composed of a set of VNFs chained together (e.g., parts of the RAN or CN elements), or a mix of Virtual Network Functions (VNFs) and Physical Network Functions (PNFs). 3GPP has put efforts  into integrating NS in the future specification of both the RAN and CN domains\cite{NS,NS2} by creating three Service and System Aspects (SA) groups in order to update the RAN, the CN, and describe a management framework for Network Slicing in 5G. The main results of these groups are: (i) the usage of a slice identifier (S-NSSAI: Single-Network Slice Selection Assistance Information), when the User Equipment (UE) first connects to the RAN; (ii) the introduction of a new CN architecture, which is virtualization-ready, and integrates a Network Slice Selection Function (NSSF) that aims to help the RAN select the CN functions corresponding to a UE’s S-NSSAI; (iii) a new framework that manages the life cycle of 5G network slices. 
% However, the End-to-end (E2E) support of Network Slicing in 5G systems given the uncertainty in the requests for slices is not explored. Moreover, while many existing solutions for the access \cite{Wireless} and E2E network slicing propose allocating a different set of physical resource blocks (PRBs) to each service in order to facilitate isolation between slices, this approach is insufficient due to the temporal changes in the channel condition.



==> IEEE NetSoft 2023 (1)/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we study the resource provisioning problem for end-to-end (E2E) network slicing under demand uncertainty. We modeled the problem as a two-stage stochastic mixed integer program (SMIP) aiming at minimizing the total resource cost over the core network (CN) and the radio access network (RAN). We develop a practical two-time-scale resource provisioning algorithm based on our SMIP model. The proposed algorithm operates in two phases with long and short time scales corresponding to the E2E resource provisioning followed by RAN resource adjustments.  We show by means of numerical simulations that the proposed algorithm successfully addresses the resource provisioning problem for network slicing under demand uncertainty. 

==> IEEE NetSoft 2023 (1)/evaluation.tex <==
\section{Performance Evaluation}
\label{sec:evaluation}
We have implemented an evaluation environment in Java, including a network slice generator and a cellular network topology generator. We use ILOG CPLEX solver interfaced with Java for embedding and solving MILP/LP models. A rectangle area of dimension $1000(m)\times1000(m)$ is considered in all the results of this section. Figure \eqref{fig:top} shows the general structure of the substrate network topology used in the experiments. It consists of 40 gNBs and 7 core nodes. The gNBs are placed randomly and a voronoi tessellation is constructed using euclidean distance to assign users to gNBs. We assume to have three different network slices, namely eMBB, URLLC and mMTC with data rate requirements showed in Tables \eqref{Slices}. All NSs have graphical architecture of Figure (1). Users are distributed according to a spatial poisson point process with mean $\lambda = 50$. The requests by users for each slice is randomly chosen. Without loss of generality, we assume that each user can request at most one NS. This is a valid assumption because if any user in the network requests for more than one slices, we can substitute it with two users each requesting one NS. 
\begin{table}[ht]
\centering
\begin{center}
\scalebox{0.9}{
\begin{tabular}{|c|c|}
\hline
\hline
Slice type & Data rate & Latency\\
\hline
eMBB & 100Mbps &\\
ULRRC & 10Mbps &\\
mMTC & 1 Mbps &\\
\hline
\hline
\end{tabular}}
\end{center}
\caption{Data rate requirements of different type of slices}
\label{Slices}
\end{table}
The performance of the SAA method is compared with a solution based the worst case scenario (\textbf{Worst}\_\textbf{MILP}) that provisions resources to serve an overloaded network with $30\%$ more network load than normal. In this case, a smaller MILP with $H=10$ is solved to find the optimal resource allocation decision. These kinds of resource overprovisioning is very close to the way todays' networks are managed in order to avoid severe service degradation in the time of pick traffic. 
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/topology.png}
  \caption{Network topology}
    \label{fig:top}
\end{figure} 
Figure \eqref{fig:time} compares the solver run time of \textbf{DET}\_\textbf{MILP} with \textbf{Worst}\_\textbf{MILP} for different number of samples. The results are averaged on $5$ generated scenarios of users distribution for each sample size. As expected, the solver run time of \textbf{DET}\_\textbf{MILP} increases when more samples are considered. Figure \eqref{fig:box} illustrates the solver run time profile for the two methods where $H=50$ samples are considered in \textbf{DET}\_\textbf{MILP} and the results are collected for 10 runs.

Figure \eqref{fig:sup} depicts the supported traffic as the number of considered samples changes. In this experiment, after the resource allocation problems \textbf{DET}\_\textbf{MILP} and \textbf{Worst}\_\textbf{MILP} are solved, a new network instance is generated and the supported traffic is computed. It can be observed that as the number of samples increases, SAA can better provision resources and the total network supported traffic can come very close to the case that an artificial overloaded network is considered for resource allocation as in \textbf{Worst}\_\textbf{MILP}. An interesting metric that can be compared in this regard is the amount of idle resources for the two methods in different network loads. Finally, the deployment cost of \textbf{Worst}\_\textbf{MILP} and \textbf{DET}\_\textbf{MILP} is compared in Figure \eqref{fig:cost} when $H=50$, which confirms that since the former allocates more resources than needed, its deployment cost increases (many allocated resources remain idle). Last but not least, it should be noted that although \textbf{Worst}\_\textbf{MILP} performs worst than \textbf{DET}\_\textbf{MILP} in terms of cost, it does not require as much as prior knowledge required by \textbf{DET}\_\textbf{MILP}, therefore, is it less sensitive to misinformation (when the actual data distribution is different from the considered distribution). Moreover, in these methods some efforts might be wasted optimizing when distribution approximation and sampling is not accurate. A future approach to reduce this bias on prior knowledge could be exploring sampling methods other than Crude Monte Carlo. Stochastic decomposition and importance sampling can be used along with the L-shaped method in order to alleviate this problem.
\begin{figure*}[t]
\begin{center}
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/time.png}
\caption{Average solver run time of \textbf{DET}\_\textbf{MILP} vs. \textbf{Worst}\_\textbf{MILP}}  
\label{fig:time}
\end{minipage} 
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/box_time.png}
  \caption{The profile of solver run time ($H = 50$ for \textbf{DET}\_\textbf{MILP})}
    \label{fig:box}
\end{minipage}\\
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/sup.png}
  \caption{Comparison of supported traffic, \textbf{DET}\_\textbf{MILP} vs. \textbf{Worst}\_\textbf{MILP}}
    \label{fig:sup}
\end{minipage}
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/cost.png}
  \caption{Comparison of deployment cost, \textbf{DET}\_\textbf{MILP} vs. \textbf{Worst}\_\textbf{MILP}}
    \label{fig:cost}
\end{minipage}
\end{center}
\end{figure*}

==> IEEE NetSoft 2023 (1)/evaluation_thesis.tex <==
\section{Performance Evaluation}
\label{sec:evaluation}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=\linewidth]{figures/setup.png}
%     \caption{Simulation Substrate Network}
%     \label{fig:eval_setup}
% \end{subfigure}
% \begin{subfigure}{0.325\textwidth}
% \centering
% \includegraphics[width=\linewidth]{figures/slice_example.png}
%   \caption{The SFC graph of mobile NSs}
%     \label{fig:slice}
%     \end{subfigure}
% \end{figure*}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\textwidth]{figures/robustness.png}
%     \caption{Relative Provisioning Cost vs. Robustness}
%     \label{fig:rob}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\textwidth]{figures/robustness.png}
%     \caption{Relative Provisioning Cost vs. Robustness}
%     \label{fig:rob}
% \end{subfigure}
% \begin{subfigure}{0.32\textwidth}
%   \includegraphics[width=\textwidth]{figures/delay_up.png}
%   \caption{UP latency}
%     \label{chapter2:delay-up}
% \end{subfigure}
% % \hspace*{\fill}
% \begin{subfigure}{0.32\textwidth}
%   \includegraphics[width=\textwidth]{figures/delay_cp.png}
%   \caption{CP latency}
%     \label{chapter2:delay-cp}
% \end{subfigure}
% \caption{UP and CP latency for URLLC, eMBB, and mMTC slices}
% \end{figure*}



% \begin{figure*}[t]
% \begin{center}
% \begin{minipage}[h]{0.325\textwidth}
% \includegraphics[width=1\linewidth]{figures/robustness.png}
% \caption{Relative cost vs. robustness}
% \label{fig:rob}
% \end{minipage}
% \begin{minipage}[h]{0.325\textwidth}
% \includegraphics[width=1\linewidth]{figures/delay_up.png}
% \caption{UP latency for different slices}
% \label{chapter2:delay-up}
% \end{minipage}
% \begin{minipage}[h]{0.325\textwidth}
% \includegraphics[width=1\linewidth]{figures/delay_cp.png}
% \caption{CP latency for different slices}
% \label{chapter2:delay-cp}
% \end{minipage}
% \end{center}
% \end{figure*}



In this section, we present the evaluation of the proposed two-timescale methodology through numerical simulations. We first describe the simulation setup and parameters and then proceed to the numerical results. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/combined_infra_ns.png}
    \caption{Example substrate (left) and NS (right)}
    \label{fig:ns-combined}
\end{figure}
% \begin{figure*}[t]
% \begin{center}
% \begin{minipage}[h]{0.4\textwidth}
% \includegraphics[width=1\linewidth]{figures/setup.png}
%     \caption{Simulation Substrate Network}
%     \label{fig:eval_setup}
% \end{minipage}
% \hspace{2em}
% \begin{minipage}[h]{0.36\textwidth}
% \includegraphics[width=1\linewidth]{figures/slice_example.png}
%   \caption{The SFC graph of mobile NSs}
%     \label{fig:slice}
% \end{minipage}
% \end{center}
% \end{figure*}
\begin{table}[t]
\centering
\caption{System Model Parameters}
\begin{center}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|}
\hline
\hline
Slice Type & $d_k^{UP}$/$d_k^{CP}$ & mean value of $\underline{R}^k_j$ & $\overline{R}^k_j$\\
\hline
\hline
eMBB (k=1) & 100/20 ms & 50 & 0.6\\
\hline
URLLC (k=2) & 25/5 ms & 10 & 0.2\\
\hline
mMTC (k=3) & 300/60 ms & 5 & 0.2\\
\hline
\end{tabular}}
\end{center}
\label{chapter2:sim_parameters}
\end{table}
\begin{figure*}[t]
\centering

\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\textwidth]{figures/delay_up.png}
  \caption{UP latency for different network slices}
    \label{chapter2:delay-up}
\end{subfigure}
% \hspace*{\fill}
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\textwidth]{figures/delay_cp.png}
  \caption{CP latency for different network slices}
    \label{chapter2:delay-cp}
\end{subfigure}
\caption{UP and CP latency for URLLC, eMBB, and mMTC slices}
\end{figure*}
\begin{figure*}[t]
\centering
\begin{subfigure}{0.32\textwidth}  \includegraphics[width=\textwidth]{figures/supported_embb.png}
  \caption{eMBB slice}
    \label{chapter2:acc-embb}
\end{subfigure}
% \end{center}
% \end{figure*}
% \begin{figure*}[t]
% \begin{center}
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\textwidth]{figures/supported_urllc.png}
  \caption{URLLC slice}
    \label{chapter2:acc-urllc}
\end{subfigure}
% \end{center}
% \end{figure*}
% \begin{figure*}[t]
% \begin{center}
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\textwidth]{figures/supported_mmtc.png}
  \caption{mMTC slice}
    \label{chapter2:acc-mmtc}
\end{subfigure}
\caption{Average request acceptance ratio for URLLC, eMBB, and mMTC slices}
\end{figure*}






\subsection{Simulation Setup}
We consider a mobile network consisting of seven general-purpose server nodes at four levels of hierarchy and $6$ gNB nodes connected to the third-level servers as illustrated in Fig. \ref{fig:ns-combined}. L1, L2, L3, and L4 servers have CPU (cycle/s), storage (GB), and RAM (GB) capacities of $(72, 144, 288)$, $(36, 72, 144)$, $(18, 36, 72)$, and $(6, 12, 24)$, respectively. The backhaul links have a capacity of $2$Gbps while the fronthaul links can support $1$Gbps of traffic. For the sake of simplicity, the resource scaling factor $\chi^\nu_k$ is assumed to be the same for all resource types $\nu \in \mathcal{T}$ and is equal to the number of users requesting slice $k$. Each VNF requires $(0.1\chi_k,0.2\chi_k,0.4\chi_k)$ units of CPU, STO, and RAM resources. The simulation environment is implemented in Java and we use the CPLEX commercial solver for solving the $\emph{DET-SMNS}$ model using the branch-and-bound method. The $\emph{RNSR}$ problem is also solved by CPLEX using the Simplex method. All experiments are carried out on an Intel Xeon processor at 2.3 GHz with 8GB memory.

We assume that the UEs are distributed in a square area with the dimension of $10\ Km\times10\ Km$. The demand density functions $\mathcal{F}^T$ are obtained by applying bivariate kernel density estimation (KDE) to the synthetic data generated for each slice demand in the considered geographical area. Due to the unavailability of spatially distributed datasets for the demand of NSs, we generate synthetic data for the UE locations using Matérn cluster point process \cite{cluster}. In this process, a number of parent points (UEs) are first generated using a Poisson point process and for each parent point (representing a cluster center), another Poisson point process is used to generate the UE distribution within a radius of the parent point. The cluster-based UE distribution represents the hot spot area for different services supported through network slices. 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/pdf_example_2.jpg}
%     \caption{Pdf}
%     \label{fig:pdf}
% \end{figure}
% It is important to note that while many statistical and analytical models have been proposed for traffic prediction in mobile network, our main focus in this chapter is the resource provisioning problem. 


We assume that the demand density functions $(\mathcal{F}^T)$ change hourly, i.e. the value of the macro-slot is one hour. Moreover, the duration of the micro-slot is set to one minute, i.e. $N_T = 60$. We consider three slices, namely, eMBB, URLLC, and mMTC with the SFC graph as depicted in Fig.~\ref{fig:ns-combined}. The simulation parameters of different NS types are given in Table \ref{chapter2:sim_parameters}.
% This parameter can be adjusted depending on the dynamicity of the considered scenario, e.g. UEs velocity and channel . 
It is worth noting that the duration of the macro-slot and micro-slot can be adjusted with respect to the slice type and the dynamicity of the considered scenario, e.g. UEs mobility parameters such as velocity, channel condition variations, etc. We use the $k$-shortest path algorithm to construct the set $\mathcal{P}( i \rightarrow j ) \forall i,j \in V$  with $k=3$. 
% Figure \ref{fig:kde_example} illustrates an example of a demand distribution for a network slice obtained by using the kernel density estimation method.
% The learned distributions are assumed to be valid estimates of the demand for the period of long time slots. 
% model which captures the hot-spots for each slice.
% \subsection{Provisioning Cost vs. Robustness}
% In this section, we evaluate the performance of the proposed solution in terms of resource provisioning cost and robustness. To this end, we first solve an instance of the $\emph{DET-SMNS}(\mathcal{H)}$ problem for a macro-slot, and then simulate $10$ realizations of the demand for different NSs and the vectors $\hat{\boldsymbol{\xi}}_i, i=1,\dots,10$. For each realization, we observe whether the obtained solution of $\emph{DET-SMNS}(\mathcal{H)}$ is a feasible solution for the realized demand. We define robustness as the percentage of the realized demands for which the obtained solution of $\emph{DET-SMNS}(\mathcal{H)}$ is feasible. We repeat this process for different values of $H$ as $1,5,10,20,30$ and in each case, average the robustness and cost over $10$ runs. Fig.~\ref{fig:rob} illustrates the relative provisioning cost and robustness as the number of sampled realization changes from $H=1$ to $H=30$. We observe that as expected, increasing the value of $H$ enhances the robustness of the solution from $77.9\%$ to $96.4\%$ at the expense of increased resource provisioning cost.
% \subsection{Performance of the Two-Timescale Solution}
% In this section, we present the performance of the proposed two-timescale resource provisioning scheme, in terms of latency and acceptance ratio. 
% We consider a duration of $60$ for short time slots and show the obtained latency and acceptance ratio for different slices. 










\subsection{Numerical Results}
Figure 4 illustrates the UP and CP latency for the URLLC, eMBB, and mMTC slices. We consider the results of $5$ and depict both the average latency and the profile of latency values for different NSs, in the cases of $H=5,10,30$. We observe that in all cases, the obtained UP and CP latencies are below the corresponding maximum tolerable latency given in Table \ref{chapter2:sim_parameters}. Thus, the proposed two-time-scale resource provisioning algorithm provides solutions that meet the NSs' QoS requirement in terms of E2E UP and CP latency. 

In Fig. 5, the average acceptance ratio of different slices averaged for the duration of $60$ micro-slots is illustrated. The percentage of accepted requests is obtained from the supported traffic solution of the \emph{RNSR} problem, and averaged over different gNBs, i.e.:
$$\text{Avg. acceptance ratio of slice $k$} = 100*\sum_{j\in V_{gNB}}\sigma^k_j/|V_{gNB}|$$  Figure \ref{chapter2:acc-embb}, \ref{chapter2:acc-urllc}, and \ref{chapter2:acc-mmtc} denote the average acceptance ratio for the eMBB, URLLC, and mMTC slices, respectively. In this experiment, we change the number of realizations from $1$ to $30$. It is observed that as the value of $H$ increases (more realizations are considered as an input to $\emph{DET-SMNS}(\mathcal{H)}$), the acceptance ratio enhances for all slices. This is due to the fact that as the number of realizations increases, the solution of the $\emph{DET-SMNS}(\mathcal{H)}$ problem is a better approximation of the original \emph{SMNS} problem modeled as a SMIP as explained in Section \ref{sec:SMNS}.




==> IEEE NetSoft 2023 (1)/formulation.tex <==
\section{System Model and Problem Formulation}
Time intervals...
A summary of the parameters is given in Table \ref{parameters}.
\label{sec:sys}
% We consider the The 5G NS resource allocation problem has two domains, the radio and the core (transport) network resource allocations. While these two problems can be solved separately, a joint approach is more sensible considering the uncertainty about demand points locations. However, obtaining the optimal decision which minimizes the overall cost is not trivial in this case. We propose a two-stage stochastic optimization framework to tackle this problem. In the following, the network and slice models are presented and then the proposed problem formulation is detailed.
\subsection{Infrastructure Network model}
Let the infrastructure network (substrate) be represented as a directed graph $G = (V, E)$, where $V$ is the set of infrastructure nodes and $E$ denotes the set of infrastructure links. The set of infrastructure network nodes consists of two type of nodes, gNB and non-gNB. Thus, $V = V_{gNB} \cup V_{-gNB}$ where $V_{gNB}$ and $V_{-gNB}$ correspond to the set of substrate gNB and non-gNB node, respectively. Each gNB is characterized by its maximum supported traffic which is computed based on its available bandwidth (physical resource blocks or PRBs) and MIMO antenna configuration. Non-gNBs are general-purpose servers providing essential capabilities for running core network functions (NFs) and could data centers. A substrate node is characterized by its available CPU, storage and RAM resources. We define the set of node resources as $\mathcal{T} = \{CPU, STO, RAM\}$. Let the vector $W_j = (W^{CPU}_j, W^{STO}_j, W^{RAM}_j)$ represent the available capacity of the substrate node $j$. These amounts correspond to the initial capacity of the node reduced by the amount allocated to previously accepted concurrent requests. Moreover, the cost of each infrastructure node $j$ being used by a VNF consists of two parts: (i) a fixed part $C_j$ paid for each VNF deployed on node $j$, (ii) a variable part associated to the per-unit usage of each resource which depends linearly on the amount of the resource consumed by a VNF. The per-unit variable cost corresponding to CPU, storage and memory of node $j$ are denoted by $C_j^{CPU}, C_j^{STO} $ and $C_j^{RAM}$. 

We assume that each gNB offers  wireless resources to MUs. The maximum traffic supported by gNB $j\in V_{gNB}$ is shown by $W^{tr}_j$. Furthermore, the set of infrastructure link $E = E_{FH} \cup E_{BH}$ where $E_{FH}$ and $E_{BH}$ stand for the links between gNB nodes and the core network and the remaining link, respectively. Each substrate link $e\in E$ has a bandwidth capacity and propagation delay denoted by $W^{BW}_e$ and $\tau^{PRO}_e$ in respective order. Moreover, a per-unit bandwidth cost is associated to the infrastructure link $e$ denoted by $C_e^{BW}$. In order to meet the traffic transmission between two VNFs of a network slice, we consider a set of substrate paths denoted by $\mathcal{P}$. 
% For the sake of simplicity, we assume that each UE is covered by one gNB and gNBs do not interfere. 

We consider an environment in which MUs submit their request for different services to SPs. For the sake of simplicity, we assume that each user requests at most one service. This can be readily extended to the case of multiple requests from a user by duplicating MUs that have multiple service requests. Each service is realized through network slices managed by SPs. The SPs meet their customers requested services by dedicating network slices with specified QoS requirements deployed on the substrate network which is owned and managed by InPs. Let $U$ denote the set of MUs distributed across the considered geographical area. We assume that each MU is served by a gNB according to the nearest association rule. 

For a user 
%and $\mathcal{K}$ and the set of network slices
% Therefore, the set of MUs served by gNB $v\in V_{gNB}$ and requesting the service met by slice $k\in \mathcal{K}$ is represented by $U_v^k$.

\subsection{Network Slice Model}
In this section, we present the network slice model. We assume that a slice request is modeled as one or multiple service function chains (SFCs), each consisting of a number of VNFs (e.g. gNB, AFM, UPF, SMF) and virtual links (VLs) between them. The set of system network slices is represented by $\mathcal{K}=\{1,...,K\}$. Let the directed graph $G^\prime_{k} = (V^\prime_{k}, E^\prime_{k})$ describe the $k$th slice' SFCs. Similarly to the substrate network, we assume that the nodes of slice $k$ consist of two types of nodes, gNB and non-gNB. Therefore, $V^\prime_{k} = V^\prime_{k,gNB} \cup V^\prime_{k,-gNB}$ where $V^\prime_{k,gNB}$ and $V^\prime_{k,-gNB}$ correspond to the set of gNBs and non-gNB functions of slice $k$. Moreover, $E^\prime_{k} =  E^\prime_{k, FH}\cup E^\prime_{k, BH}$ where $E^\prime_{k, FH}$ and $E^\prime_{k, BH}$ denote the fronthaul and backhaul VLs, respectively. 
We assume that each instance of the SFC corresponding to slice $k$ has QoS requirements expressed as gNB's spectrum $r_k$ and maximum E2E acceptable latency $d_k$. In addition, each VNF instance of the node $j^\prime$ in slice $k$ requires the CPU, storage and RAM resources, represented by the vector $R_{j^\prime}= (R^{CPU}_{j^\prime}, R^{STO}_{j^\prime}, R^{RAM}_{j^\prime})$. Similarly, each VL $e^\prime \in E^\prime_{k}$ is characterized by the bandwidth requirement of $R^{BW}_{e^\prime}$ to meet the demand for data transmission between the two end-pints (VNFs) of $e^\prime$. We assume that the traffic flow of each $e^\prime \in E^\prime_k$ is routed through substrate paths. Therefore, we represent the set of substrate paths considered for slice $k$ edges by $\mathcal{P}_k$, where $\mathcal{P}_k \subseteq \mathcal{P}$.

In order to satisfy the demands of all users requesting a network slice, multiple instances of that slice may be required to be deployed. We define the parameter $u_v^{k,i}$ which is equal to $1$ if user $i$ of slice $k$ is covered by gNB $v$ and $0$ otherwise. Moreover, the parameter $I_k$ indicates the number of instances of slice $k$ needed to be deployed in order to support the demand for slice $k$. Due to the mobility of the MUs and their varying demands, the true values of $u_v^{k,i}$ and $I_k$ are not known. However, given the historical data on the demand and mobility patterns of MUs, the SP and InP are capable of estimating the statistical characteristics of $u_v^{k,i}$ and $I_k$. We assume that at each time instance, the spatial distribution of demand points for different network slices are given, represented by $\mathcal{F}_1,\dots,\mathcal{F}_k, k\in \mathcal{K}$. Hence, $u_v^{k,i}$ and $I_k$ become random variables with known distributions. Define $\mathcal{F} = \{\mathcal{F}_1,\dots,\mathcal{F}_k\}, k\in \mathcal{K}$.
%**** In order to speed up the reconfiguration process and minimize VNF migrations resulted from users mobility and change of covering gNB, we assume that all instances of the core VNFs for a NS are embedded on one substrate node in contrast to the virtual gNBs that are essentially placed on different substrate gNBs as required. 
\begin{figure}[!t]
\centering
\includegraphics[width=0.35\textwidth]{figures/slice.png}
  \caption{A network slice example}
    \label{fig:slice}
\end{figure}
\begin{table*}[t]
\centering
\begin{center}
\scalebox{1}{
\begin{tabular}{c|c}
\hline
\hline
Network Parameters & Description\\
\hline
$G = (V, E)$ & The substrate network graph\\
$V_{gNB}, V_{core}$ & The set of substrate RAN and core nodes\\
$E_{FH}, E_{BH}$ & The set of fronthaul and backhaul links\\
$W_{v}^{tr}$ & maximum traffic rate supported by gNB $v$\\
$U^k$ & Number of users of slice $k$ in the network\\
$W_j^{CPU,STO,RAM}$ & The amount of CPU, Storage, and RAM capacities of the substrate node $j$\\
$W_e^{CAP}$ & The capacity of the substrate link $e$\\
\hline
\hline
Slice Parameters & Description\\
\hline
$K$ & Number of requested slices\\
$G^k_{slc} = (V_{slc}^k, E_{slc}^k)$& The $k$th slice SFC graph\\
$V^k_{slc,ran}, V^k_{slc,core}$ & the set of virtual RAN and core VNFs\\
$E_{slc, FH}^k, E_{slc, BH}^k$ & The set of fronthaul and backhaul virtual links\\
$r_k$ & slice $k$ rate requirement\\
$R_{j^\prime}^{CPU, STO, RAM}$ & The amount of CPU, Storage and RAM resource requirements of the VNF $j^{\prime}$\\
$R_{e^\prime}^{CAP}$ & The data rate requirement of the virtual link $e^\prime$\\
\hline
\hline
\end{tabular}}
\end{center}
\caption{System model parameters}
\label{parameters}
\end{table*}

\subsection{Problem formulation}
% Figure \ref{fig:architecture} illustrates an example of E2E resource allocation for different slices. 
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/architecture.png}
%   \caption{An example of the E2E slice resource allocation}
%     \label{fig:architecture}
% \end{figure} 
% The problem architecture is illustrated at the bottom of this figure.
%The main consideration is that the problem is solved for a set of gNBs connected to a single gateway acting as an aggregation point. 
Given the substrate network and network slice graphs, we formulate the problem of E2E network slicing under demand uncertainty as a two-stage SMIP, using the following variables:
\begin{itemize}
\item A set of binary variables $\boldsymbol{x}_{k}$ where $x_j^{k,j^\prime}$ is $1$ if the an instance of VNF $j^\prime$ of the $k$th slice is placed at substrate node $j$.
\item A set of binary variables $\boldsymbol{y}_{k}$ where $y_p^{k,e^\prime}$ is 1 if the virtual link $e^\prime$ of the $k$th slice is assigned to substrate path $p$.
\item A set of continuous decision variables $\boldsymbol{z}_k$ where $z_j^k$ represents the fraction of gNB $j$ supported traffic that is allocated to slice $k$.
\end{itemize}
It is important to note that the value of the vector $\boldsymbol{z} = (z_1^1,...,z_{|V_{gNB}|}^1,...,z_1^K,...,z_{|V_{gNB}|}^K)$ represents the RAN slicing policy defined as the fraction of each cell available spectrum that is assigned to each requested slice. For example, in the case of having three network slices, the subsequent RAN slice allocation for a gNB can be $20\%, 50\% $, and $30\%$. Once this spectrum assignment policy is determined, the actual radio resource allocation in terms of the number of PRBs allocated to the users of each slice to fulfill the spectrum requirement is formulated separately. In this regard, different solutions have been proposed in the literature with the goal of minimizing the interference between different mobile virtual network operators \cite{RAN}. 

We model the resource provisioning problem for the requested slices as a two-stage SMIP. We refer to this method as \textbf{SMIP} which is described in the following sections.

\subsubsection{First-stage problem}
The first-stage objective in \textbf{SMIP} is the minimization of the total provisioning cost which consists of node and link deployment costs for all slices. Let $\mathcal{C}_k^{N}$ and $\mathcal{C}_k^{L}$ denote the node and link costs corresponding to slice $k$, respectively. Consequently, we have:
% \begin{strip}
\begin{equation}
    \mathcal{C}_k^N(\boldsymbol{x}_{k}) = \sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}C_j^kx_{j}^{k}+\sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}\sum_{t\in \mathcal{T}}R_{j^\prime}^tC_j^t x_j^{k,j^\prime}
    \label{SMIP:node-cost}
\end{equation}
\begin{equation}
    \mathcal{C}_k^L(\boldsymbol{y}_{k}) = \sum_{p\in\mathcal{P}}\sum_{e\in p}\sum_{e^\prime \in E^\prime_k} R_{e^\prime}^{BW} C_e^k y_{p}^{k, e^\prime}
    \label{SMIP:link-cost}
\end{equation}
% +\phi_2\sum_{e\in E}\sum{e^\prime \in E^\prime_k} z_{e}^{k, e^\prime} C_e^k) +\phi_3\mathbb{E} Q_{x,z}(u)
where
\begin{equation}
  x_{j}^{k} =
    \begin{cases}
      1 & \text{if $\sum_{j^\prime\in V^\prime_{k}}x_j^{k,j^\prime} \geq 0$}\\
      0 & \text{otherwise}
    \end{cases}       
\end{equation}
Hence, the first-stage objective is: \begin{equation}
     \mathcal{C}_1 (\boldsymbol{x},\boldsymbol{y}) = \phi_1\sum_{k\in\mathcal{K}}\mathcal{C}^N_k(\boldsymbol{x}_k)+\phi_2 \sum_{k\in\mathcal{K}}\mathcal{C}^L_k(\boldsymbol{y}_k)
     \label{SMIP:Obj1}
\end{equation}
where $\phi_1$ and $\phi_2$ are constants to balance between the two objective terms of \eqref{SMIP:node-cost} and \eqref{SMIP:link-cost}.
% +\phi_3\mathbb{E} Q_{x,y}(U)

For each infrastructure node and link, we have capacity constraints as follows:
\begin{equation}
    \text{C1}:\ \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} I_k \leq W_j^{t} \quad t\in \mathcal{T}, \forall j\in V_{} \label{SIMP:node-Cap1}
\end{equation}
\begin{equation}
    \text{C2}:\ \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} I_k \leq W_e^{BW} \quad \forall e \in E
    \label{SIMP:link-Cap1}
\end{equation}
Moreover, in a feasible resource provisioning solution, each gNB VNF is placed at one substrate gNB node and each non-gNB VNF runs on a substrate non-gNB node. Thus, the resulting VNFs deployment must guarantee the following constraints:
% \begin{equation}
%     \text{C3}:\ \sum_{j\in V_{gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,gNB}
%     \label{SIMP:gNB-map1} -->removed
% \end{equation}
\begin{equation}
    \text{C3}:\ \sum_{j\in V_{-gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,-gNB}
    \label{SIMP:non-gNB-map1}
\end{equation}
Let $\mathcal{P}^\prime_k$ denote the set of all paths of slice $k \in \mathcal{K}$. The execution latency of VNF $j^\prime \in V^\prime_k$ on the infrastructure node is represented by $\tau^{k,j^\prime}$. Given the edge mapping decision variables $y^{k,e^\prime}_p$, the data transmission latency corresponding to the infrastructure edge $e\in E$ based on its aggregated assigned data demand is computed in equation \eqref{d-edge}.
\begin{equation}
    \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e} \label{d-edge}
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ mapped to the path $p\in \mathcal{P}_k$ is:
\begin{equation}
    \sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ is computed in equation \eqref{d-slice-edge}.
\begin{equation}
    \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \label{d-slice-edge}
\end{equation}
The latency of slice $k$ instances experienced by the MUs of that slice is guaranteed to be lower than the required latency of the slice in constraints \eqref{SIMP:latency-1}.
\begin{align}
    & \text{C4}: \nonumber\\
    & \sum_{e^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \right]\nonumber\\
    & + \sum_{j^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \right]  \leq d_k\quad \forall p^\prime \in \mathcal{P}^{\prime}_k, k\in \mathcal{K} \label{SIMP:latency-1}
\end{align}
Finally, the domain constraints are presented as follows:
\begin{align}
    & \text{C5}: 
    x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \ k\in \mathcal{K}, j\in V, j^\prime \in V^\prime_k, p\in \mathcal{P}_k, e^\prime \in E^\prime_k \label{SMIP:dom1}
\end{align}
% \begin{align}
%&\textbf{s.t} \nonumber \\
%& \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% &\sum_{e\in\delta^+(j)} z_{e}^{k, e^\prime} - \sum_{e\in\delta^-(j)}z_{e}^{k, e^\prime} = 
    %\left\{
    %\begin{array}{@{}ll@{}}
    %1 & if \quad j = destination(e^\prime)\\
    %-1 &  if \quad j = source(e^\prime)\\
    %0 & otherwise\\
    %\end{array}\right. \quad k=1,...,K, \forall j \in V, e^\prime \in E^k_{slc} \label{path}\\
% &\sum_{k=1}^K \sum_{j^\prime\in V_{slc}^k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \leq W_j^{t} \quad t\in \{CPU, STO, RAM\}, \forall j\in V_{} \label{node_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,FH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{FH}\label{link_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,BH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{BH}\label{link_cap2}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{}\label{link_cap1}\\
% &\sum_{j\in V_{core}}x_{j}^{k,j^\prime} = 1 \quad k=1,...,K, \forall j^\prime \in V^k_{slc,core} \label{placement1}\\
% & x_j^{k, j^\prime}\in \{0,1\}, z_{e}^{k,e^\prime} \geq 0  \quad k = 1,...,K, j\in V, j^{\prime}\in V^{k}_{slc}, e\in E, e^\prime \in E^k_{slc} \label{domain1}
% \end{align} 
% \end{strip}

%%second stage
\subsubsection{Second-stage problem} The goal of the second-stage problem is to minimize the total gNB traffic allocated to network slices. 
The second-stage objective is:
\begin{equation}
     \mathcal{C}_2(\boldsymbol{z}) = \sum_{k\in\mathcal{K}}\sum_{j\in V_{gNB}} z^k_{j}
\end{equation}
The flow conservation constraints are guaranteed by equations \eqref{SIMP:flow2-nongNB} and \eqref{SIMP:flow2-gNB}.  
\begin{align}
    & \text{C6}:\ \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_{k} \nonumber\\
    &\qquad\qquad\forall k\in\mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{SIMP:flow2-nongNB}
\end{align}
\begin{align}
    & \text{C7}:\ \sum_{\substack{p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\  j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} - y_{q(j \rightarrow i)}^{k,e^\prime} = x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime} \nonumber \\
    &\qquad\qquad \forall k\in \mathcal{K}, i\in V_{gNB}, e^\prime(i^\prime \rightarrow j^\prime)\in E_{k,FH}^\prime \label{SIMP:flow2-gNB}
\end{align}
The traffic allocated to the users of a slice must be greater than the required traffic of slice k. This constraint is ensured by equations \eqref{SIMP:reqrate}.
\begin{align}
    & \text{C8}:\ z_j^k W_j^{tr} \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\ 
    & \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
\end{align}
% \begin{align}
%     & \text{C8}:\ c k_i (1-BER_i) \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\
%     &\quad \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
% \end{align}
The capacity constraint of gNBs is enforced by equation \eqref{SIMP:gNBcap}. 
% \begin{equation}
%     \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq W_j^{tr} \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
% \end{equation}
\begin{equation}
    % \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
    \text{C9}:\ \sum_{k=1}^K z_{j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
\end{equation}
The gNB placement constraints are enforced by equation \eqref{SIMP:gNBplacement2}.
\begin{equation}
    \text{C10}: \ x_j^{k, j^\prime} = \mathbbm{1}_{\{\sum_{i=1}^{U_k} u_{i,j}^k\geq1\}} \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:gNBplacement2}\\
\end{equation}
The domain constraints of the second-stage problem are:
\begin{align}
    & \text{C11}: \ z^k_j \in [0, 1] \quad \forall k\in \mathcal{K}, j\in V_{gNB},  \label{domain2} 
\end{align}
% Let $Q(\boldsymbol{x},\boldsymbol{y}, U)$ denote the optimal value of the second-stage problem. 
The E2E network slicing problem with demand uncertainties is formulated as a two-stage SMIP presented below:
\begin{align}
    & {minimize} \quad \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) + \eta \ \mathbb{E}_{
    \mathcal{F}} [min \ \mathcal{C}_2 (\boldsymbol{z})] \label{SMIP:obj} \\
    & \qquad \qquad \qquad \text{s.t.}  \qquad \text{C1}-\text{C11} \nonumber
\end{align}
% $Q_{x,z}(u)$ is the optimal value of the second-stage defined as follows:
% \begin{strip}
% \begin{align}
% &\textbf{minimize}
% \quad \sum_{k=1}^{K} (\sum_{v\in V_{gNB}} z_k^v) \label{obj2}\\
% &\textbf{s.t} \nonumber \\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{j}^{k,m}-x_{j}^{k,n})I_{k} \quad k = 1,...,K, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path2}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% & y_k^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{U_k} r_k u_{k,i}^v \quad k =1,...,K, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate}\\
% &\sum_{k=1}^K y_k^v \leq W_v^{tr} \quad \forall v\in V_{gNB} \label{cap_ran}\\
%&\sum_{}z_{e}^{e^\prime , k}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{U_k} u_{i,k}^j\geq1\}} \quad k = 1..., K, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement2}\\
% & y_k^v \in [0, W_v^{tr}], \quad k = 1..., K, \forall  v\in V_{gNB},  \label{domain2}
% \end{align}
% \end{strip}
The objective \eqref{SMIP:obj} minimizes the summation of the core slice provisioning cost and the expectation of the second stage objective which is the RAN slice provisioning cost. $\eta$ is a constant parameter that determines the balance between the objectives of the first and second stages.
% The constraint sets \eqref{node_cap1} and \eqref{link_cap1} ensure that the demand allocated to each substrate core node and fronthaul link does not exceed its capacity. The constraint set \eqref{link_cap2} ensures that the demand allocated to each substrate backhaul link does not exceed its capacity. Constraint \eqref{placement1} guarantees that each core VNF is placed at one core substrate node. Finally, the domain constraints are expressed in \eqref{domain1}.The second stage problem objective in \eqref{obj2} minimizes the BW consumption. Constraint \eqref{path2} and  \eqref{path1} enforce the existence of a path in the substrate network for each virtual backhaul and fronthaul link. Constraint \eqref{rate} guarantees that the rate of gNB $v$ allocated to slice $k$ to be greater than the total demand of the users covered by $v$. Constraint \eqref{cap_ran} limits the load allocated to a gNB to the maximum traffic that can be supported by the gNB. Constraint \eqref{placement2} ensures that a virtual gNB of slice $k$ is placed at a gNB if at least one user of that slice is covered by that gNB. The domain constraints for the second-stage problem is expressed by \eqref{domain2}.



==> IEEE NetSoft 2023 (1)/formulation2.tex <==
\section{System Model and Problem Formulation}
We consider the resource provisioning problem of mobile network slicing across both RAN and core components. In this section, the network and slice models are presented followed by problem formulation.
\label{sec:sys}
% We consider the The 5G NS resource allocation problem has two domains, the radio and the core (transport) network resource allocations. While these two problems can be solved separately, a joint approach is more sensible considering the uncertainty about demand points locations. However, obtaining the optimal decision which minimizes the overall cost is not trivial in this case. We propose a two-stage stochastic optimization framework to tackle this problem. In the following, the network and slice models are presented and then the proposed problem formulation is detailed.
\subsection{Infrastructure Network model}
Let the infrastructure network (substrate) be represented as a directed graph $G = (V, E)$, where $V$ is the set of infrastructure nodes and $E$ denotes the set of infrastructure links. The set of infrastructure network nodes consist of two type of nodes, gNB and non-gNB. Thus, $V = V_{gNB} \cup V_{-gNB}$ where $V_{gNB}$ and $V_{-gNB}$ correspond to the set of substrate gNB and non-gNB node, respectively. Each gNB is characterized by its maximum supported traffic which is computed based on its available bandwidth (physical resource blocks or PRBs) and MIMO antenna configuration. Non-gNBs are general-purpose servers providing essential capabilities for running core network network functions (NFs) and could data centers. A substrate node is characterized by its available CPU, storage and RAM resources. We define the set of node resources as $\mathcal{T} = \{CPU, STO, RAM\}$. Let the vector $W_j = (W^{CPU}_j, W^{STO}_j, W^{RAM}_j)$ represent the available capacity of the substrate node $j$. These amounts correspond to the initial capacity of the node reduced by the amount allocated to previously accepted concurrent requests. Moreover, the cost of each infrastructure node $j$ being used by a VNF consist of two parts: (i) a fixed part $C_j$ paid for each VNF deployed on node $j$, (ii) a variable part associated to the per-unit usage of each resource which depends linearly on the amount of the resource consumed by a VNF. The per-unit variable cost corresponding to CPU, storage and memory of node $j$ are denoted by $C_j^{CPU}, C_j^{STO} $ and $C_j^{RAM}$. 

We assume that the available
spectrum of gNB $j\in V_{gNB}$ is divided into a set of $W^{RAN}_j$ physical resource blocks (PRBs)  can be allocate to different users of different slices \cite{} \cite{papa2021user}. Furthermore, the set of infrastructure link $E = E_{FH} \cup E_{BH}$ where $E_{FH}$ and $E_{BH}$ stand for the links between gNB nodes and the core network and the remaining link, respectively. Each substrate link $e\in E$ has a bandwidth capacity and propagation delay denoted by $W^{BW}_e$ and $\tau^{PRO}_e$ in respective order. Moreover, a per-unit bandwidth cost is associated to the infrastructure link $e$ denoted by $C_e^{BW}$. In order to meet the traffic transmission between two VNFs of a network slice, we consider a set of substrate paths denoted by $\mathcal{P}$. Let $\mathcal{P}( i \rightarrow j )$ denote the set of substrate path between $i$ and $j$. Therefore, $\mathcal{P} = \cup_{i,j\in V, i\neq j} \mathcal{P}( i \rightarrow j )$.
% For the sake of simplicity, we assume that each UE is covered by one gNB and gNBs do not interfere. 

We consider an environment in which MUs submit their request for different services to SPs. For the sake of simplicity, we assume that each user requests at most one service. This can be readily extended to the case with multiple requests from a user by duplicating MUs which have multiple service requests. Each service is realized through network slices managed by SPs. The SPs meet their customers requested services by dedicating network slices with specified QoS requirements deployed on the substrate network which is owned and managed by InPs. Let $U$ denoted the set of MUs distributed across the considered geographical area. We assume that each MU is served by a gNB according to the nearest association rule. 

For a user 
%and $\mathcal{K}$ and the set of network slices
% Therefore, the set of MUs served by gNB $v\in V_{gNB}$ and requesting the service met by slice $k\in \mathcal{K}$ is represented by $U_v^k$.


\subsection{Network Slice Model}
In this section, we present the network slice model. We assume that a slice request is modeled as one or multiple service function chains (SFCs), each consisting of a number of VNFs (e.g. gNB , AFM, UPF, SMF) and virtual links (VLs) between them. The set of system network slices is represented by $\mathcal{K}=\{1,...,K\}$. Let the directed graph $G^\prime_{k} = (V^\prime_{k}, E^\prime_{k})$ describe the $k$th slice' SFCs. Similarly to the substrate network, we assume that the nodes of slice $k$ consists of two types of nodes, gNB and non-gNB. Therefore, $V^\prime_{k} = V^\prime_{k,gNB} \cup V^\prime_{k,-gNB}$ where $V^\prime_{k,gNB}$ and $V^\prime_{k,-gNB}$ correspond to the set of gNBs and non-gNB functions of slice $k$. Moreover, $E^\prime_{k} =  E^\prime_{k, FH}\cup E^\prime_{k, BH}$ where $E^\prime_{k, FH}$ and $E^\prime_{k, BH}$ denote the fronthaul and backhaul VLs, respectively. 
We assume that each instance of the SFC corresponding to slice $k$ has QoS requirements expressed as gNB's radio resource $r_k$ and maximum E2E tolerable latency $d_k$. In addition, each VNF instance of the node $j^\prime$ in slice $k$ requires the CPU, storage and RAM resources, represented by the vector $R_{j^\prime}= (R^{CPU}_{j^\prime}, R^{STO}_{j^\prime}, R^{RAM}_{j^\prime})$. Similarly, each VL $e^\prime \in E^\prime_{k}$ is characterized by the bandwidth requirement of $R^{BW}_{e^\prime}$ to meet the demand for data transmission between the two end-pints (VNFs) of $e^\prime$. We assume that the traffic flow of each $e^\prime \in E^\prime_k$ is routed through substrate paths. Therefore, we represent the set of substrate paths considered for slice $k$ edges by $\mathcal{P}_k$, where $\mathcal{P}_k \subseteq \mathcal{P}$.

In order to satisfy the demands of all users requesting a network slice, multiple instances of that slice may be required to be deployed. We define the parameter $u_v^{k,i}$ which is equal to $1$ if user $i$ of slice $k$ is covered by gNB $v$ and $0$ otherwise. Moreover, the parameter $I_k$ indicates the number of instances of slice $k$ needed to be deployed in order to support the demand for slice $k$. Due to the mobility of the MUs and their varying demands, the true values of $u_v^{k,i}$ and $I_k$ are not known. However, given the historical data on the demand and mobility patterns of MUs, the SP and InP are capable of estimating the statistical characteristics of $u_v^{k,i}$ and $I_k$. 
%**** In order to speed up the reconfiguration process and minimize VNF migrations resulted from users mobility and change of covering gNB, we assume that all instances of the core VNFs for a NS are embedded on one substrate node in contrast to the virtual gNBs that are essentially placed on different substrate gNBs as required. 
\begin{figure}[!t]
\centering
\includegraphics[width=0.30\textwidth]{figures/slice_example.png}
  \caption{A network slice example}
    \label{fig:slice}
\end{figure}
\begin{table*}[t]
\centering
\begin{center}
\scalebox{1}{
\begin{tabular}{c|c}
\hline
\hline
Network Parameters & Description\\
\hline
$G = (V, E)$ & Substrate network graph\\
$V_{gNB}, V_{core}$ & Set of substrate gNB and non-gNB nodes\\
% $E_{FH}, E_{BH}$ & The set of fronthaul and backhaul links\\
$\mathcal{P}$ & Set of Substrate paths\\
$W_{v}^{tr}$ & Available spectrum of gNB $v$\\
$U^k$ & Number of users of slice $k$ in the network\\
$W_j^{CPU,STO,RAM}$ & The amount of CPU, Storage and RAM capacities of the substrate node $j$\\
$W_e^{CAP}$ & The capacity of the substrate link $e$\\
\hline
\hline
Slice Parameters & Description\\
\hline
$K$ & Number of requested slices\\
$G^k_{slc} = (V_{slc}^k, E_{slc}^k)$& The $k$th slice SFC graph\\
$V^k_{slc,ran}, V^k_{slc,core}$ & the set of virtual RAN and core VNFs\\
$E_{slc, FH}^k, E_{slc, BH}^k$ & The set of fronthaul and backhaul virtual links\\
$r_k$ & slice $k$ rate requirement\\
$R_{j^\prime}^{CPU, STO, RAM}$ & The amount of CPU, Storage and RAM resource requirements of the VNF $j^{\prime}$\\
$R_{e^\prime}^{CAP}$ & The data rate requirement of the virtual link $e^\prime$\\
\hline
\hline
\end{tabular}}
\end{center}
\caption{System model parameters}
\label{parameters}
\end{table*}

\begin{itemize}
\item $I_k$: number of virtual gNBs supported by slice $k$ core (not a random variable)
\item $\chi_k$: scaling factor of BW, compute and storage resources for slice $k$
\end{itemize}
\subsection{Two-timescale resource reservation framework}
%change the sentences! is directly form another paper
We assume the lifecycle of resource management for the considered network slices is set to be one day. The reason that we choose the resource management lifecycle of a slice as one
day is because this lifecycle exhibits the property of periodicity.
The user traffic may vary during different time of the day. The
variation of user traffic may follow a certain pattern during the
day. We divide 24 hours into $Q$ long timescale slots (minutes). We assume that at long time slot $q$, the spatial distribution of demand points for $K$ different network slices are given, represented by $\mathcal{F}_1,\dots,\mathcal{F}_k, k\in \mathcal{K}$. Hence, $u_v^{k,i}$ and $I_k$ become random variables with known distributions. Define $\mathcal{F}^q = \{\mathcal{F}_1^q,\dots,\mathcal{F}_k^q\}, k\in \mathcal{K}$.
Each long timescale slot consists of $T$ short timescale slots
with the same duration. Resource reservation for the considered
slice is updated at the beginning of each long timescale slot
with the statistical knowledge of user traffic. Intra-slice resource
allocation is performed over short timescale under an arbitrary
user arrival/departure process. The choice of the duration of each
long timescale slot should guarantee that the statistics of user
\subsection{Problem formulation}
% Figure \ref{fig:architecture} illustrates an example of E2E resource allocation for different slices. 
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/architecture.png}
%   \caption{An example of the E2E slice resource allocation}
%     \label{fig:architecture}
% \end{figure} 
% The problem architecture is illustrated at the bottom of this figure.
%The main consideration is that the problem is solved for a set of gNBs connected to a single gateway acting as an aggregation point. 
Given the substrate network and network slice graphs, we formulate the problem of E2E network slicing under demand uncertainty as a two-stage SMIP, using the following variables:
\begin{itemize}
\item A set of binary variables $\boldsymbol{x}_{k}$ where $x_j^{k,j^\prime}$ is $1$ if the an instance of VNF $j^\prime$ of the $k$th slice is placed at substrate node $j$.
\item A set of binary variables $\boldsymbol{y}_{k}$ where $y_p^{k,e^\prime}$ is 1 if the virtual link $e^\prime$ of the $k$th slice is assigned to substrate path $p$.
\item A set of continuous decision variables $\boldsymbol{z}_k$ where $z_j^k$ represents the fraction of gNB $j$ supported traffic that is allocated to slice $k$.
\end{itemize}
It is important to note that the value of the vector $\boldsymbol{z} = (z_1^1,...,z_{|V_{gNB}|}^1,...,z_1^K,...,z_{|V_{gNB}|}^K)$ represents the RAN slicing policy defined as the fraction of each cell available radio resource that is assigned to each requested slice. For example, in the case of having three network slices, the resulted RAN slice allocation for an gNB can be $20\%, 50\% $ and $30\%$. Once this spectrum assignment policy is determined, the actual radio resource allocation in terms of the number of PRBs allocated to the users of each slice to fulfill the spectrum requirement is formulated separately. In this regard, different solutions have been proposed in the literature with the goal of minimizing the interference between different mobile virtual network operators \cite{RAN}. 

We model the resource provisioning problem for the requested slices as a two-stage SMIP. We refer to this method as \textbf{SMIP} which is described in the following sections.

\subsubsection{First-stage problem}
The first-stage objective in \textbf{SMIP} is the minimization of the total provisioning cost which consists of node and link deployment costs for all slices. Let $\mathcal{C}_k^{N}$ and $\mathcal{C}_k^{L}$ denote the node and link costs corresponding to slice $k$, respectively. Consequently, we have:
% \begin{strip}
\begin{equation}
    \mathcal{C}_k^N(\boldsymbol{x}_{k}) = \sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}C_j^kx_{j}^{k}+\sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}\sum_{t\in \mathcal{T}}R_{j^\prime}^tC_j^t x_j^{k,j^\prime}
    \label{SMIP:node-cost}
\end{equation}
\begin{equation}
    \mathcal{C}_k^L(\boldsymbol{y}_{k}) = \sum_{p\in\mathcal{P}}\sum_{e\in p}\sum_{e^\prime \in E^\prime_k} R_{e^\prime}^{BW} C_e^k y_{p}^{k, e^\prime}
    \label{SMIP:link-cost}
\end{equation}
% +\phi_2\sum_{e\in E}\sum{e^\prime \in E^\prime_k} z_{e}^{k, e^\prime} C_e^k) +\phi_3\mathbb{E} Q_{x,z}(u)
where
\begin{equation}
  x_{j}^{k} =
    \begin{cases}
      1 & \text{if $\sum_{j^\prime\in V^\prime_{k}}x_j^{k,j^\prime} \geq 0$}\\
      0 & \text{otherwise}
    \end{cases}       
\end{equation}
Hence, the first-stage objective is: \begin{equation}
     \mathcal{C}_1 (\boldsymbol{x},\boldsymbol{y}) = \phi_1\sum_{k\in\mathcal{K}}\mathcal{C}^N_k(\boldsymbol{x}_k)+\phi_2 \sum_{k\in\mathcal{K}}\mathcal{C}^L_k(\boldsymbol{y}_k)
     \label{SMIP:Obj1}
\end{equation}
where $\phi_1$ and $\phi_2$ are constants to balance between the two objective terms of \eqref{SMIP:node-cost} and \eqref{SMIP:link-cost}.
% +\phi_3\mathbb{E} Q_{x,y}(U)

For each infrastructure node and link, we have capacity constraints as follows:
\begin{equation}
    \text{C1}:\ \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \chi_k \leq W_j^{t} \quad t\in \mathcal{T}, \forall j\in V_{} \label{SIMP:node-Cap1}
\end{equation}
\begin{equation}
    \text{C2}:\ \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} \chi_k \leq W_e^{BW} \quad \forall e \in E
    \label{SIMP:link-Cap1}
\end{equation}
Moreover, in a feasible resource provisioning solution, each gNB VNF is placed at one substrate gNB node and each non-gNB VNF runs on a substrate non-gNB node. Thus, the resulting VNFs deployment must guarantee the following constraints:
% \begin{equation}
%     \text{C3}:\ \sum_{j\in V_{gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,gNB}
%     \label{SIMP:gNB-map1} -->removed
% \end{equation}
\begin{equation}
    \text{C3}:\ \sum_{j\in V_{-gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,-gNB}
    \label{SIMP:non-gNB-map1}
\end{equation}
Let $\mathcal{P}^\prime_k$ denote the set all paths of slice $k \in \mathcal{K}$. The execution latency of VNF $j^\prime \in V^\prime_k$ on infrastructure node is represented by $\tau^{k,j^\prime}$. Given the edge mapping decision variables $y^{k,e^\prime}_p$, the data transmission latency corresponding to the infrastructure edge $e\in E$ based on its aggregated assigned data demand is computed in equation \eqref{d-edge}.
\begin{equation}
    \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e} \label{d-edge}
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ mapped to the path $p\in \mathcal{P}_k$ is:
\begin{equation}
    \sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ is computed in equation \eqref{d-slice-edge}.
\begin{equation}
    \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \label{d-slice-edge}
\end{equation}
The latency of slice $k$ instances experienced by the MUs of that slice is guaranteed to be lower than the required latency of the slice in constraints \eqref{SIMP:latency-1}.
\begin{align}
    & \text{C4}: \nonumber\\
    & \sum_{e^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \right]\nonumber\\
    & + \sum_{j^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \right]  \leq d_k\quad \forall p^\prime \in \mathcal{P}^{\prime}_k, k\in \mathcal{K} \label{SIMP:latency-1}
\end{align}
Finally, the domain constraints are presented as follows:
\begin{align}
    & \text{C5}: 
    x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \ k\in \mathcal{K}, j\in V, j^\prime \in V^\prime_k, p\in \mathcal{P}_k, e^\prime \in E^\prime_k \label{SMIP:dom1}
\end{align}
% \begin{align}
%&\textbf{s.t} \nonumber \\
%& \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% &\sum_{e\in\delta^+(j)} z_{e}^{k, e^\prime} - \sum_{e\in\delta^-(j)}z_{e}^{k, e^\prime} = 
    %\left\{
    %\begin{array}{@{}ll@{}}
    %1 & if \quad j = destination(e^\prime)\\
    %-1 &  if \quad j = source(e^\prime)\\
    %0 & otherwise\\
    %\end{array}\right. \quad k=1,...,K, \forall j \in V, e^\prime \in E^k_{slc} \label{path}\\
% &\sum_{k=1}^K \sum_{j^\prime\in V_{slc}^k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \leq W_j^{t} \quad t\in \{CPU, STO, RAM\}, \forall j\in V_{} \label{node_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,FH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{FH}\label{link_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,BH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{BH}\label{link_cap2}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{}\label{link_cap1}\\
% &\sum_{j\in V_{core}}x_{j}^{k,j^\prime} = 1 \quad k=1,...,K, \forall j^\prime \in V^k_{slc,core} \label{placement1}\\
% & x_j^{k, j^\prime}\in \{0,1\}, z_{e}^{k,e^\prime} \geq 0  \quad k = 1,...,K, j\in V, j^{\prime}\in V^{k}_{slc}, e\in E, e^\prime \in E^k_{slc} \label{domain1}
% \end{align} 
% \end{strip}
The flow conservation constraints are guaranteed by equations \eqref{SIMP:flow2-nongNB} and \eqref{SIMP:flow2-gNB}.  
\begin{align}
    & \text{C6}:\ \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime} \nonumber\\
    &\qquad\qquad\forall k\in\mathcal{K},  e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{SIMP:flow2-nongNB}
\end{align}
\begin{align}
    & \text{C7}:\ \sum_{\substack{p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\  j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} - y_{q(j \rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_{k} \nonumber \\
    &\qquad\qquad \forall k\in \mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime \rightarrow j^\prime)\in E_{k,FH}^\prime \label{SIMP:flow2-gNB}
\end{align}

%%second stage
\subsubsection{Second-stage problem} The goal of the second-stage problem is to minimize the total gNB traffic allocated to network slices. 
The second-stage objective is:
\begin{equation}
     \mathcal{C}_2(\boldsymbol{z}) = \sum_{k\in\mathcal{K}}\sum_{j\in V_{gNB}} z^k_{j}
\end{equation}
% \begin{align}
%     & \text{C8}:\ c k_i (1-BER_i) \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\
%     &\quad \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
% \end{align}
The traffic allocated to the users of a slice must be greater than the required traffic of slice k. This constraint is ensured by equations \eqref{SIMP:reqrate}.
\begin{align}
    & \text{C8}:\ z_j^k W_j^{RAN} \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\ 
    & \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
\end{align}
\begin{align}
    & \text{C8:} \frac{\sum_{i=1}^{U_k}u^k_{i,j}}{\sum_{k=1}^K\sum_{i=1}^{U_k}u^k_{i,j}} \leq z^k_j\ \forall j\in V_{gNB} \label{SIMP:reqrate}
\end{align}
The capacity constraint of gNBs is enforced by equation \eqref{SIMP:gNBcap}. 
% \begin{equation}
%     \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq W_j^{tr} \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
% \end{equation}
\begin{equation}
    % \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
    \text{C9}:\ \sum_{k=1}^K z_{j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
\end{equation}
The gNB placement constraints are enforced by equation \eqref{SIMP:gNBplacement2}.
\begin{equation}
    \text{C10}: \ x_j^{k, j^\prime} = \mathbbm{1}_{\{\sum_{i=1}^{U_k} u_{i,j}^k\geq1\}} \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:gNBplacement2}\\
\end{equation}
The domain constraints of the second-stage problem are:
\begin{align}
    & \text{C11}: \ z^k_j \in [0, 1] \quad \forall k\in \mathcal{K}, j\in V_{gNB},  \label{domain2} 
\end{align}
% Let $Q(\boldsymbol{x},\boldsymbol{y}, U)$ denote the optimal value of the second-stage problem. 
The E2E network slicing problem with demand uncertainties is formulated as a two-stage SMIP presented below:
\begin{align}
    & {minimize} \quad \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) + \eta \ \mathbb{E}_{
    \mathcal{F}} [min \ \mathcal{C}_2 (\boldsymbol{z})] \label{SMIP:obj} \\
    & \qquad \qquad \qquad \text{s.t.}  \qquad \text{C1}-\text{C11} \nonumber
\end{align}
% $Q_{x,z}(u)$ is the optimal value of the second-stage defined as follows:
% \begin{strip}
% \begin{align}
% &\textbf{minimize}
% \quad \sum_{k=1}^{K} (\sum_{v\in V_{gNB}} z_k^v) \label{obj2}\\
% &\textbf{s.t} \nonumber \\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{j}^{k,m}-x_{j}^{k,n})I_{k} \quad k = 1,...,K, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path2}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% & y_k^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{U_k} r_k u_{k,i}^v \quad k =1,...,K, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate}\\
% &\sum_{k=1}^K y_k^v \leq W_v^{tr} \quad \forall v\in V_{gNB} \label{cap_ran}\\
%&\sum_{}z_{e}^{e^\prime , k}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{U_k} u_{i,k}^j\geq1\}} \quad k = 1..., K, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement2}\\
% & y_k^v \in [0, W_v^{tr}], \quad k = 1..., K, \forall  v\in V_{gNB},  \label{domain2}
% \end{align}
% \end{strip}
The objective \eqref{SMIP:obj} minimizes the summation of the core slice provisioning cost and the expectation of the second stage objective which is the RAN slice provisioning cost. $\eta$ is a constant parameter which determines the balance between the objectives of the first and second stages.
% The constraint sets \eqref{node_cap1} and \eqref{link_cap1} ensure that the demand allocated to each substrate core node and fronthaul link does not exceed its capacity. The constraint set \eqref{link_cap2} ensures that the demand allocated to each substrate backhaul link does not exceed its capacity. Constraint \eqref{placement1} guarantees that each core VNF is placed at one core substrate node. Finally, the domain constraints are expressed in \eqref{domain1}.The second stage problem objective in \eqref{obj2} minimizes the BW consumption. Constraint \eqref{path2} and  \eqref{path1} enforce the existence of a path in the substrate network for each virtual backhaul and fronthaul link. Constraint \eqref{rate} guarantees that the rate of gNB $v$ allocated to slice $k$ to be greater than the total demand of the users covered by $v$. Constraint \eqref{cap_ran} limits the load allocated to a gNB to the maximum traffic that can be supported by the gNB. Constraint \eqref{placement2} ensures that a virtual gNB of slice $k$ is placed at a gNB if at least one user of that slice is covered by that gNB. The domain constraints for the second-stage problem is expressed by \eqref{domain2}.



==> IEEE NetSoft 2023 (1)/formulation_thesis.tex <==
\section{Problem Formulation}
\label{sec:formulation_thesis}
In this section, we formulate the E2E network slicing problem under demand uncertainty as a two-stage SMIP. Before we present the problem formulation, in the next subsection we provide a brief overview of stochastic programming \cite{book}. 

\subsection{Stochastic Programming}
\label{sec:prelim}
\textit{Stochastic linear programs} (SLPs) are linear programs where some data are uncertain, represented as random variables with given probability measures. The values of these random variables are only known after a realization of a random experiment. SLP optimization decision variables are classified into two groups: first-stage variables, determined before conducting the experiment, and second-stage variables, determined after the experiment outcome is observed.
% The value of the random variables are known only after a random experiment. Hence, the set of optimization decision variables in SLP are divided into two groups: (i) first-stage decision variables, (ii) second-stage decision variables. While the first-stage variables are determined before the random experiment, the second-stage decisions are taken after the random experiment becomes known. 
Let $\boldsymbol{x} \in \mathbb{R}^{n_1\times 1}$ denote the vector of first-stage optimization variables. Define the random variable corresponding to the unknown data as $\boldsymbol{\xi}=\boldsymbol{\xi}(\omega)$ with $\omega\in \Omega$ representing a random outcome. The vector of second-stage decision variables is denoted by $\boldsymbol{y}(\omega,\boldsymbol{x})$. We assume that the probability distribution $\mathcal{F}$ on $\Omega$ is known in the first stage. The classical two-stage SLP with \textit{fixed recourse} is formulated as follows:
\begin{align}
    & minimize \quad \boldsymbol{c}^T \boldsymbol{x} + \mathbb{E}_{\mathcal{F}}[min\ \boldsymbol{q}(\omega)^T \boldsymbol{y}(\omega,\boldsymbol{x})] \label{SLP-obj}\\
    & s.t. \quad A\boldsymbol{x} = \boldsymbol{b}\label{SLP-c1}\\
    & T(\omega)\boldsymbol{x} + W \boldsymbol{y}(\omega,\boldsymbol{x}) = \boldsymbol{h}(\omega)\label{SLP-c2}\\
    & \boldsymbol{x},\boldsymbol{y}(\omega,\boldsymbol{x}) \geq \boldsymbol{0} \label{SLP-c3}.
\end{align}
where $\boldsymbol{c}\in \mathbb{R}^{n_1\time 1}, \boldsymbol{b}\in \mathbb{R}^{m_1\times 1}, A\in \mathbb{R}^{m_1\times n_1}$. The objective function \eqref{SLP-obj} consists of the deterministic term $\boldsymbol{c}^T \boldsymbol{x}$ and the expectation of the term $\boldsymbol{q}(\omega)^T \boldsymbol{y}(\omega,\boldsymbol{x})$ over all realizations $\omega$. Note that once $\omega$ is realized, $T(\omega) \in \mathbb{R}^{m_2\times n_2}, \boldsymbol{h}(\omega) \in \mathbb{R}^{m_2\times 1}$, and $\boldsymbol{q}(\omega)\in \mathbb{R}^{n_2\times 1}$ become known. In particular $\boldsymbol{\xi}(\omega) = (\boldsymbol{q}(\omega), \boldsymbol{h}(\omega), T_1(\omega),\dots,T_{m_2}(\omega))$ represents the random data vector where $T_1(\omega),\dots,T_{m_2}(\omega)$ are the rows of $T(\omega)$. For a given $\omega$, let $Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))$ denote the value of the second-stage problem, defined as:
{
\begin{align}
    & Q(\boldsymbol{x},\boldsymbol{\xi}(\omega)) = min_{\boldsymbol{y}\geq 0} \{\boldsymbol{q}(\omega)^T \boldsymbol{y} | W\boldsymbol{y} = \boldsymbol{h}(\omega)-T(\omega)\boldsymbol{x}\} \label{2-stage-value}
\end{align}
}

Moreover, the expected value of the second-stage objective value is defined as:
\begin{align}
    & \mathcal{Q}(\boldsymbol{x}) = \mathbb{E}_{\mathcal{F}}[Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))] \label{2-stage-expected-value}
\end{align}
The \textit{deterministic equivalent program} (DEP) corresponding to \eqref{SLP-obj}-\eqref{SLP-c3} is defined as:
\begin{align}
    & min \quad \boldsymbol{c}^T \boldsymbol{x} + \mathcal{Q}(\boldsymbol{x}) \label{DEP-obj}\\
    & s.t. \quad A\boldsymbol{x} = \boldsymbol{b} \label{DEP-c1}\\
    & \boldsymbol{x} \geq \boldsymbol{0} \label{DEP-c2}
\end{align}
The DEP formulation illustrates the major difference between a deterministic linear program and an SLP. Given $\mathcal{Q}(\boldsymbol{x})$, an SLP is an ordinary nonlinear program due to the nonlinearity of $\mathcal{Q}(\boldsymbol{x})$. On the other hand, the computation of $\mathcal{Q}(\boldsymbol{x})$ requires evaluating $Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))$ for all $\boldsymbol{x}$ and $\omega$ that is not possible in practice. The problem becomes even more challenging considering the first-stage or second-stage variables to be integers, i.e. $\boldsymbol{x}\in \mathbb{Z}^{n_1}$, $\boldsymbol{y}\in \mathbb{Z}^{n_2}$. Next, we present our proposed formulation for the network slicing problem under demand uncertainty, which is based on two-stage stochastic mixed-integer programming. 







\subsection{ Stochastic Mobile Network Slicing Optimization Model}
\label{sec:SMNS}
We start by defining the decision variables for the optimization model as follows:
\begin{itemize}
\item $\boldsymbol{x}_{k}$: the set of binary variables where $x_j^{k,j^\prime}$ is equal to $1$ if the VNF $j^\prime$ of the $k$th slice is placed on the substrate node $j$.
\item $\boldsymbol{y}_{k}$: the set of binary variables where $y_p^{k,e^\prime}$ is equal to $1$ if the VL $e^\prime$ of the $k$th slice is mapped to substrate path $p\in\mathcal{P}_k$.
\item $\boldsymbol{z}_k$: the set of continuous variables where $z_j^k$ represents the fraction of gNB $j$ spectrum allocated to slice $k$.
\end{itemize}
The vector $\boldsymbol{z} = (z_1^1,...,z_{|V_{gNB}|}^1,...,z_1^K,...,z_{|V_{gNB}|}^K)$ represents the RAN slicing policy defined as the fraction of residual radio resource at each cell that is assigned to each slice. For instance, in the case of having three NSs, the resulting RAN slice allocation for a gNB can be $20\%, 50\% $, and $30\%$. Once this spectrum assignment policy is determined, the actual radio resource allocation in terms of the scheduled PRBs for the users of each slice is obtained from a separate problem that is out of the scope of this paper. In this regard, different solutions have been proposed in the literature. For instance, authors in \cite{RAN} proposed a RAN resource allocation solution given the spectrum assignment policy, with the objective of minimizing the interference between different mobile virtual network operators. 

We model the resource provisioning problem for the requested slices as a two-stage SMIP. We refer to this problem as stochastic mobile network slicing (\emph{SMNS}). The two stages of the problem are explained in the following.

\subsubsection{First-Stage Problem}
The first-stage objective of \emph{SMNS} is the minimization of the total provisioning cost which consists of node and link deployment costs for all slices. Let $\mathcal{C}_k^{N}$ and $\mathcal{C}_k^{L}$ denote the node and link costs corresponding to slice $k$, respectively. Consequently, we have:
% \begin{strip}
\begin{equation}
    \mathcal{C}_k^N(\boldsymbol{x}_{k}) = \sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}} C_j^kx_{j}^{k}+\sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}\sum_{\nu\in \mathcal{T}}\gamma_\nu R_{j^\prime}^\nu C_j^\nu x_j^{k,j^\prime}
    \label{SMIP:node-cost}
\end{equation}
\begin{equation}
    \mathcal{C}_k^L(\boldsymbol{y}_{k}) = \sum_{p\in\mathcal{P}}\sum_{e\in p}\sum_{e^\prime \in E^\prime_k}\gamma_{BW} R_{e^\prime}^{BW} C_e^{BW} y_{p}^{k, e^\prime}
    \label{SMIP:link-cost}
\end{equation}
% +\phi_2\sum_{e\in E}\sum{e^\prime \in E^\prime_k} z_{e}^{k, e^\prime} C_e^k) +\phi_3\mathbb{E} Q_{x,z}(u)
where
\begin{equation}
  x_{j}^{k} =
    \begin{cases}
      1 & \text{if $\sum_{j^\prime\in V^\prime_{k}}x_j^{k,j^\prime} \geq 0$}\\
      0 & \text{otherwise}
    \end{cases}       
\end{equation}

Hence, the first-stage objective is: \begin{equation}
     \mathcal{C}_1 (\boldsymbol{x},\boldsymbol{y}) = \sum_{k\in\mathcal{K}}\mathcal{C}^N_k(\boldsymbol{x}_k)+ \sum_{k\in\mathcal{K}}\mathcal{C}^L_k(\boldsymbol{y}_k)
     \label{SMIP:Obj1}
\end{equation}
where $\gamma_\nu, \nu\in\mathcal{T}\cup\{BW\}$ are the weights used to balance the objective terms of \eqref{SMIP:Obj1} corresponding to different resources.
% +\phi_3\mathbb{E} Q_{x,y}(U)
In a valid network slicing solution, each gNB VNF is placed at substrate gNB nodes only and each non-gNB VNF runs on a substrate non-gNB node. Thus, the resulting VNFs deployment must satisfy the following constraints:
\begin{equation}
    \sum_{j\in V_{-gNB}}x_j^{k,j^\prime} = 1, \ \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,-gNB}
    \label{SIMP:non-gNB-map1}
\end{equation}
\begin{equation}
    x_j^{k,j^\prime} = 0, \ \forall k \in \mathcal{K},j\in V_{-gNB}, j^\prime \in V^\prime_{k,gNB}
    \label{SIMP:gNB-map1} 
\end{equation}
% \begin{align}
%&\textbf{s.t} \nonumber \\
%& \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% &\sum_{e\in\delta^+(j)} z_{e}^{k, e^\prime} - \sum_{e\in\delta^-(j)}z_{e}^{k, e^\prime} = 
    %\left\{
    %\begin{array}{@{}ll@{}}
    %1 & if \quad j = destination(e^\prime)\\
    %-1 &  if \quad j = source(e^\prime)\\
    %0 & otherwise\\
    %\end{array}\right. \quad k=1,...,K, \forall j \in V, e^\prime \in E^k_{slc} \label{path}\\
% &\sum_{k=1}^K \sum_{j^\prime\in V_{slc}^k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \leq W_j^{t} \quad t\in \{CPU, STO, RAM\}, \forall j\in V_{} \label{node_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,FH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{FH}\label{link_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,BH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{BH}\label{link_cap2}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{}\label{link_cap1}\\
% &\sum_{j\in V_{core}}x_{j}^{k,j^\prime} = 1 \quad k=1,...,K, \forall j^\prime \in V^k_{slc,core} \label{placement1}\\
% & x_j^{k, j^\prime}\in \{0,1\}, z_{e}^{k,e^\prime} \geq 0  \quad k = 1,...,K, j\in V, j^{\prime}\in V^{k}_{slc}, e\in E, e^\prime \in E^k_{slc} \label{domain1}
% \end{align} 
% \end{strip}
The flow conservation is guaranteed by constraints \eqref{SIMP:flow2-nongNB} and \eqref{SIMP:flow2-gNB}, 
\begin{align}
    & \sum_{\substack{{}p \in \mathcal{P}_k (i\rightarrow j)\\q \in \mathcal{P}_k (j\rightarrow i)\\ j\in V}} y_{p}^{k,e^\prime} -y_{q}^{k,e^\prime} = x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime},\nonumber \\ 
    & \forall k\in\mathcal{K}, e^\prime \in E^\prime_{k,BH}, src(e^\prime) = i^\prime, dst(e^\prime) = j^\prime \label{SIMP:flow2-nongNB}
\end{align}
\begin{align}
    & \sum_{\substack{p \in \mathcal{P}_k(i\rightarrow j)\\ q\in \mathcal{P}_k(j\rightarrow i) \\ j\in V}} y_{p}^{k,e^\prime} - y_{q}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_{k},\nonumber \\ 
    &\forall k\in \mathcal{K}, i\in V_{-gNB}, e^\prime\in E_{k,FH}^\prime, src(e^\prime) = i^\prime, dst(e^\prime) = j^\prime \label{SIMP:flow2-gNB} 
\end{align}
The domain constraints are as follows,
{\small
\begin{align}
    & x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\}  \ \forall k\in \mathcal{K}, j\in V, j^\prime \in V^\prime_k, p\in \mathcal{P}_k, e^\prime \in E^\prime_k \label{SMIP:dom1}
\end{align}
}
%%second stage
\subsubsection{Second-Stage Problem} The goal of the second-stage problem is to minimize the total cost of gNBs' radio resources allocated to different NSs. 
The second-stage objective is:
\begin{equation}
     \mathcal{C}_2(\boldsymbol{z}) = \sum_{k\in\mathcal{K}}\sum_{j\in V_{gNB}} C^k_j z^k_{j} W^r_j
\end{equation}
% \begin{align}
%     & \text{C8}:\ c k_i (1-BER_i) \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\
%     &\quad \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
% \end{align}
% The traffic allocated to the users of a slice must be greater than the required traffic of slice k. This constraint is ensured by equations \eqref{SIMP:reqrate}.
% \begin{align}
%     & \text{C8}:\ z_j^k W_j^{RAN} \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\ 
%     & \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
% \end{align}
% If $x^{k,j^\prime}_j x^{l,j^\prime}_j = 1, j^\prime\in V^\prime_{k,gNB}$:
% \begin{align}
%     & \text{C8:}\ \frac{\sum_{i=1}^{U_k}u^k_{i,j}}{\sum_{k=1}^K\sum_{i=1}^{U_k}u^k_{i,j}} \leq z^k_j\ \forall j\in V_{gNB}, k\in\mathcal{K} \label{SIMP:reqrate}
% \end{align}
%%%%%%%RAN slicing policy: 
%1-balancing:
% Moreover, provisioning of spectrum resources has to be performed in a balanced way, consistent with the slice demands \cite{agg}. We assume that when a gNB serves users requesting different network slices, the amount of provisioned spectrum for each slice is as the same proportion as the corresponding demand. This resource proportionality constraint is formulated as:
% \begin{align}
%     & \text{C8:}\nonumber\\ 
%     & \frac{1}{\sum_{i=1}^{U_{k_1}}u^{k_1}_{i,j}}z^{k_1}_j = \frac{1}{\sum_{i=1}^{U_{k_2}}u^{k_2}_{i,j}}z^{k_2}_j = \dots = \frac{1}{\sum_{i=1}^{U_{k_{\sigma(j)}}}u^{k_{\sigma(j)}}_{i,j}}z^{k_{\sigma(j)}}_j \nonumber\\
%     &\qquad \forall j\in V_{gNB}, k_l \in \mathcal{K}, \sum_{i=1}^{U_{{k_l}}}u^{{k_l}}_{i,j}\geq 0, l=1,\dots,\sigma(j) \label{SIMP:reqrate}
% \end{align}
% where $\sigma(j)$ is the number of slices to be served by gNB $j\in V_{gNB}$.
%%%%%%%%%%%


%%%%balanced with stupid formulation
% \begin{align}
%     & \text{C8:}\ x^{k,j^\prime}_j x^{l,j^\prime}_j((\sum_{i=1}^{U_k}u^k_{i,j})z^l_j - (\sum_{i=1}^{U_l}u^l_{i,j})z^k_j) = 0 \nonumber\\
%     &\quad \forall j\in V_{gNB},j^\prime\in V^\prime_{k,gNB}, j^\prime\in V^\prime_{l,gNB}, \ k,l \in \mathcal{K}, k\neq l \label{SIMP:reqrate}
% \end{align}
% Equation \eqref{SIMP:reqrate} is equivalent to the following:
% \begin{align}
%     & \text{C8:}\ (\sum_{i=1}^{U_k}u^k_{i,j})z^l_j - (\sum_{i=1}^{U_l}u^l_{i,j})z^k_j \leq (2-x^{k,j^\prime}_j-x^{l,j^\prime}_j) M \nonumber\\
%     &\qquad  (\sum_{i=1}^{U_k}u^k_{i,j})z^l_j - (\sum_{i=1}^{U_l}u^l_{i,j})z^k_j \geq (x^{k,j^\prime}_j+x^{l,j^\prime}_j-2)M \nonumber\\
%     &\quad \forall j\in V_{gNB},j^\prime\in V^\prime_{k,gNB}, k,l \in \mathcal{K}, k\neq l \label{SIMP:reqrate}
% \end{align}

The processing delay of VNF $j^\prime \in V^\prime_k$ on an infrastructure node is represented by $\tau^{k,j^\prime}$. Given the VL mapping decision variables $y^{k,e^\prime}_p$, the data transmission latency corresponding to the infrastructure edge $e\in E$ given its aggregated load is calculated as:
\begin{equation}
    \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{\chi_{k}^{BW}R^{BW}_{e^\prime}}{W^{BW}_e} \label{d-edge} \nonumber
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ mapped to the path $p\in \mathcal{P}_k$ is:
\begin{equation}
    \sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{\chi_{k}^{BW}R^{BW}_{e^\prime}}{W^{BW}_e}\right] \nonumber
\end{equation}
Therefore, the latency of VL $e''$ is calculated as follows:
\begin{equation}
    \sum_{p\in\mathcal{P}_k} y^{k,e''}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{\chi_{k}^{BW}R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \label{d-slice-edge} \nonumber
\end{equation}
% which is equal to $ \sum_{p\in\mathcal{P}_k}  \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right]$ since $(y^{k,e^\prime}_p)^2 = y^{k,e^\prime}_p$. 
Thus, the maximum UP/CP latency of slice $k$ instances are guaranteed to be lower than the required latency $d^{UP}_k$/$d^{CP}_k$ in the following constraint:
{\small
\begin{align}
    & \sum_{e'' \in p^\prime} \left[ \sum_{p\in\mathcal{P}_k} y^{k,e''}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{\chi_{k}^{BW}R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \right] \nonumber\\
    &+ \sum_{j^\prime \in p^\prime} \left[ \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \right]  \leq d_k^{UP/CP}, \forall p^\prime \in \mathcal{P}^{\prime}_{k,UP/CP}, k\in \mathcal{K} \nonumber
\end{align}}
The above constraint ensures that the maximum latency of each slice is less than its tolerable latency by enforcing the inequality for all paths of $G^\prime_k$. By doing so, the latency over the \textit{critical path} defined as the path inducing the maximum latency among all paths is enforced to be less than the tolerable latency. This constraint is a quadratic constraint. Thus, we linearize it by introducing a set of additional  continuous variables $\eta_p \geq 0$ and $\eta_p^{k,e^\prime} \geq 0$, defined as the latency of path $p\in\mathcal{P}$ and the latency of VL $e^\prime \in E^\prime_k$ of slice $k$ on path $p$, respectively. Therefore, the latency constraint is converted to the following set of constraints:
{
\begin{align}
    & \sum_{e\in q}\left[ \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p} \sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p\frac{\chi_{k}^{BW}R^{BW}_{e^\prime}}{W^{BW}_e}\right] = \eta_q, \ \forall q\in \mathcal{P} \label{SIMP:latency-1}
\end{align}
}
\begin{align}
    &\zeta y^{k,e^\prime}_p + \eta_p - \eta^{k,e^\prime}_p \leq \zeta, \ \forall p\in\mathcal{P}_k, e^\prime \in E^\prime_k, k\in\mathcal{K}\label{SIMP:latency-2}
\end{align}
\begin{align}
    &\sum_{e^\prime \in p^\prime} \sum_{p\in \mathcal{P}_k} \eta^{k,e^\prime}_p + \sum_{j^\prime \in p^\prime} \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \leq d^{UP/CP}_k,\nonumber \\ &\forall p^\prime \in \mathcal{P}^\prime_{k,UP/CP}, k\in \mathcal{K} \label{SIMP:latency-3}
\end{align}
where $\zeta$ is a large real constant. We also add the term $\epsilon \mathcal{D}$ to the objective function where $\mathcal{D}(\boldsymbol{\eta})=\sum_{k\in \mathcal{K}}\sum_{p\in \mathcal{P}_k}\sum_{e^\prime\in E^\prime_k}\eta_p^{k,e^\prime}$ and $\epsilon$ is a very small value in order to make sure that the main objective of minimizing the resource provisioning cost is not affected by adding $\mathcal{D}$. By doing so, it is ensured that the value of $\eta_p^{k,e^\prime}$ is positive if and only if $y_p^{k,e^\prime} = 1$. 
% Hence,
% \begin{equation}
%      \mathcal{C}_2 (\boldsymbol{z},\boldsymbol{\eta_p},\boldsymbol{\eta}) = \sum_{k\in\mathcal{K}}\mathcal{C}^N_k(\boldsymbol{x}_k)+ \sum_{k\in\mathcal{K}}\mathcal{C}^L_k(\boldsymbol{y}_k)+\epsilon\mathcal{D}
%      \nonumber
% \end{equation}

%%%%RAN slicing with translator
% Let $\underline{R}^k_j$ denote the average required minimum and number of PRBs to be allocated to a user of slice $k\in \mathcal{K}$ in gNB $j\in V_{gNB}$. Similar to \cite{8624268}, we assume that the network-level performance requirement of a slice $k\in \mathcal{K}$ can be translated into the cell-level radio resource requirements $\underline{R}^k_j$ represented by the required number of radio resources. $\underline{R}^k_j$ may be determined based on the radio channel quality between users and the serving gNB to support the throughout requirements of the requested network slice.
Given the network-level performance translation to cell-level metric $\underline{R}^k_j$, the RAN slice resource allocation is enforced by the following constraints:
\begin{equation}
     \sum_{i=1}^{U_k}u_{j}^{k,i}\underline{R}^k_j \leq x^{k,j^\prime}_j z^k_{j}W^r_j, \ \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
\end{equation}
Constraints \eqref{SIMP:reqrate} is nonlinear due to the term $x^{k,j^\prime}_j z^k_{j}W^r_j$. We use the big-M method and convert \eqref{SIMP:reqrate} to the following:
\begin{align}
     & \sum_{i=1}^{U_k}u_{j}^{k,i}\underline{R}^k_j \leq z^k_{j}W^r_j+(1-x^{k,j^\prime}_j)M, \ \forall k\in\mathcal{K}, \nonumber\\
     & j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate-bigM}
\end{align}
where $M\in\mathbb{R}$ is a large number. Moreover, in order to satisfy the slice isolation constraint and given the maximum allowable number of PRBs allocated to each slice at each gNB, $\overline{R}^k_j$, we formulate the slice isolation constraint using the following inequality:
\begin{equation}
    z^k_{j}W^r_j \leq \overline{R}^k_j x^{k,j^\prime}_j, \ \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:isolation}
\end{equation}
Moreover, for each infrastructure node and link, we have capacity constraints as follows:
\begin{equation}
    \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^\nu \chi_k^\nu \leq W_j^\nu, \ \nu\in \mathcal{T}, \forall j\in V_{} \label{SIMP:node-Cap1}
\end{equation}
\begin{equation}
    \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} \chi_k^{BW} \leq W_e^{BW},\ \forall e \in E
    \label{SIMP:link-Cap1}
\end{equation}
% if $\sum_k z^k_j = 1$
Furthermore, the capacity constraint of gNB $j\in V_{gNB}$ is enforced by the following inequality: 
% \begin{equation}
%     \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq W_j^{tr} \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
% \end{equation}
\begin{equation}
    % \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
    \sum_{k=1}^K z_{j}^k = x^{k,j^\prime}_j,\ \forall j\in V_{gNB}, j^\prime \in  V_{k,gNB}^\prime \label{SIMP:gNBcap}\\
\end{equation}
The gNB placement constraint is enforced by the following:
\begin{equation}
    x_j^{k, j^\prime} \geq \mathbbm{I}{\{\sum_{i=1}^{U_k} u_{j}^{k,i}\geq1\}},\ \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:gNBplacement2}\\
\end{equation}
Finally, the domain constraints of the second-stage problem are:
\begin{align}
    & z^k_j \in [0, 1],\ \forall k\in \mathcal{K}, j\in V_{gNB}\nonumber\\ 
    & \eta^{k,e^\prime}_p, \eta_p \geq 0,\ \forall k\in \mathcal{K}, e^\prime \in E^\prime_k, p\in \mathcal{P}_k \label{domain2} 
\end{align}

% \subsection{Stochastic Mobile Network Slicing}
The E2E network slicing problem with demand uncertainty is formulated as a two-stage SMIP presented below:
\begin{align}
    & {minimize} \ \phi_1\mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) + \phi_2 \ \mathbb{E}_{
    \boldsymbol{\xi}} [min \ \mathcal{C}_2 (\boldsymbol{z})+\epsilon \mathcal{D(\boldsymbol{\eta})}] \label{SMIP:obj} \\
    & \qquad \qquad \qquad \text{s.t.}  \qquad \eqref{SIMP:non-gNB-map1}-\eqref{domain2} \nonumber
\end{align}

% $Q_{x,z}(u)$ is the optimal value of the second-stage defined as follows:
% \begin{strip}
% \begin{align}
% &\textbf{minimize}
% \quad \sum_{k=1}^{K} (\sum_{v\in V_{gNB}} z_k^v) \label{obj2}\\
% &\textbf{s.t} \nonumber \\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{j}^{k,m}-x_{j}^{k,n})I_{k} \quad k = 1,...,K, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path2}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% & y_k^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{U_k} r_k u_{k,i}^v \quad k =1,...,K, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate}\\
% &\sum_{k=1}^K y_k^v \leq W_v^{tr} \quad \forall v\in V_{gNB} \label{cap_ran}\\
%&\sum_{}z_{e}^{e^\prime , k}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{U_k} u_{i,k}^j\geq1\}} \quad k = 1..., K, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement2}\\
% & y_k^v \in [0, W_v^{tr}], \quad k = 1..., K, \forall  v\in V_{gNB},  \label{domain2}
% \end{align}
% \end{strip}
The objective \eqref{SMIP:obj} minimizes the summation of the core slice provisioning cost and the expectation of the second stage objective which is the RAN slice provisioning cost. The weights $\phi_1,\phi_2$ determine the balance between the objectives of the first and second stage problems. An interpretation of the \emph{SMNS} is as follows: 
\begin{itemize}
    \item The InP provisions the core network resources for different NSs, represented by the decision variables $\boldsymbol{x}, \boldsymbol{y}$, before the actual value of the random vector 
    \begin{align}
    & \boldsymbol{\xi}=(\mathcal{U}_1, \dots, \mathcal{U}_K, u^{1,1}_{1}, \dots, u^{1,{U}_1}_{1}, \dots, u^{K,\mathcal{U}_K}_{|V_{gNB}|},\nonumber\\ 
    &\chi^\nu_1, \dots, \chi^\nu_K, \nu\in \mathcal{T}\cup\{BW\}) \nonumber
    \end{align} is realized.
    \item After the realization of $\boldsymbol{\xi}$, the RAN resource provisioning and delay decision variables, denoted by $\boldsymbol{z,\eta}$, are determined.
\end{itemize}
The expectation term in \eqref{SMIP:obj} requires an integration over the high-dimensional random vector $\boldsymbol{\xi}$. To tackle this challenge, we use the sample average approximation technique and replace the expectation in \eqref{SMIP:obj} with its sample average approximation (SAA). The samples can be viewed as historical observed data or can be generated using Monte Carlo sampling techniques.
% The constraint sets \eqref{node_cap1} and \eqref{link_cap1} ensure that the demand allocated to each substrate core node and fronthaul link does not exceed its capacity. The constraint set \eqref{link_cap2} ensures that the demand allocated to each substrate backhaul link does not exceed its capacity. Constraint \eqref{placement1} guarantees that each core VNF is placed at one core substrate node. Finally, the domain constraints are expressed in \eqref{domain1}.The second stage problem objective in \eqref{obj2} minimizes the BW consumption. Constraint \eqref{path2} and  \eqref{path1} enforce the existence of a path in the substrate network for each virtual backhaul and fronthaul link. Constraint \eqref{rate} guarantees that the rate of gNB $v$ allocated to slice $k$ to be greater than the total demand of the users covered by $v$. Constraint \eqref{cap_ran} limits the load allocated to a gNB to the maximum traffic that can be supported by the gNB. Constraint \eqref{placement2} ensures that a virtual gNB of slice $k$ is placed at a gNB if at least one user of that slice is covered by that gNB. The domain constraints for the second-stage problem is expressed by \eqref{domain2}.
\subsection{Deterministic Equivalent Reformulation}
\label{sec:DEF}
In this section, we introduce the deterministic reformulation of the modeled \emph{SMNS} and then propose a solution based on the SAA. The SAA method is an approach for solving stochastic optimization problems by using Monte Carlo simulation. Suppose that $H$ i.i.d observations of the random variables $u_{j}^{k,i}$, $U_k$, and $\chi_k^\nu$ are available, denoted by $\tilde{u}_{j,h}^{k,i}$,$\Tilde{U}_{k,h}$, $\Tilde{\chi}^\nu_{k,h}$, $h = 1,\dots,H$. For each realization, we define a separate set of second-stage decision variables $z_{j,h}^k, \eta_{p,h}, \eta_{p,h}^{k,e^\prime}$. Thus, we convert \emph{SMNS} to its sampled deterministic equivalent problem, defined as follows:
% \begin{strip}

\begin{align}
% \begin{gather*}
% &{minimize} \quad \medmath{\sum_{k=1}^{K} \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) +\phi_3 \sum_{h=1}^H p_h \mathcal{C}_2(\boldsymbol{z}_h)}
% \label{obj_det} \\
&{minimize} \quad \phi_1\mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) +\phi_2 \sum_{h=1}^H \frac{1}{H} \left( \mathcal{C}_2(\boldsymbol{z}_h) + \epsilon \mathcal{D}(\boldsymbol{\eta}_h)\right)
\label{obj_det} 
\end{align}

\begin{align}
    &{subject \text{ }to:}\quad\quad\quad\quad\quad\quad\eqref{SIMP:non-gNB-map1} - \eqref{SMIP:dom1}\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\nonumber
\end{align}
% \begin{align}
% % &{s.t.} \qquad \qquad \qquad \text{C3,C4, C5}, \text{C6,C7}
% &{s.t.} \qquad \eqref{SIMP:non-gNB-map1} - \eqref{SMIP:dom1} \nonumber
% \end{align}
\begin{align}
& \sum_{e\in q}\left[ \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p} \sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p\frac{\tilde{\chi}_{k,h}^{BW}R^{BW}_{e^\prime}}{W^{BW}_e}\right] - \eta_{q,h} = 0, \nonumber\\
&\forall q\in \mathcal{P},h\in\mathcal{H} \label{DET-latency-1}
\end{align}
\begin{align}
& \zeta y^{k,e^\prime}_p + \eta_{p,h} - \eta^{k,e^\prime}_{p,h} \leq \zeta, \ \forall p\in\mathcal{P}_k, e^\prime \in E^\prime_k, k\in\mathcal{K}, h\in \mathcal{H}\label{DET-latency-2}
\end{align}
\begin{align}
& \sum_{e^\prime \in p^\prime} \sum_{p\in \mathcal{P}_k} \eta^{k,e^\prime}_{p,h} + \sum_{j^\prime \in p^\prime} \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \leq d^{UP/CP}_k,\nonumber\\
&\forall p^\prime \in \mathcal{P}^\prime_{k,UP/CP}, k\in \mathcal{K}, h\in \mathcal{H} \label{DET-latency-3}
\end{align}
\begin{align}
& \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{\nu} \tilde{\chi}^\nu_{k,h} \leq W_j^{\nu},\ \forall \nu\in \mathcal{T}, j\in V_{}, h\in\mathcal{H} \label{DET-cap1}
\end{align}
{
\begin{align}
& \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} \tilde{\chi}^{BW}_{k,h} \leq W_e^{BW},\nonumber\\& \forall e \in E, h\in\mathcal{H} \label{DET-cap2}
\end{align}
}
\begin{align}
% & \text{C14}: \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_k \nonumber\\
% &\forall k\in\mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{path1_det}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{i}^{k,m}-x_{i}^{k,n})\hat{I}_{k,h} \quad k = 1,...,K, h=1,...,H, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path1_det}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path2_det}\\
% & \text{C15}: \ z_{j,h}^k W_j^{tr} \geq x^{k,j^\prime}_j\sum_{i = 1}^{\hat{U}_{k,h}} r_k \hat{u}_{i,j,h}^k \nonumber \\
% &\forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in\mathcal{H} \label{rate_det}\\
% & \text{C15}: \frac{1}{\sum_{i=1}^{\tilde{U}_{k_1,h}}\tilde{u}^{k_1}_{i,j,h}}z^{k_1}_{j,h} = \dots = \frac{1}{\sum_{i=1}^{\tilde{U}_{k_{\sigma(j)},h}}\tilde{u}^{k_{\sigma(j)}}_{i,j,h}}z^{k_{\sigma(j)}}_{j,h} \nonumber\\
% &\forall j\in V_{gNB}, k_l \in \mathcal{K}, \sum_{i=1}^{\tilde{U}_{{k_l}}}\tilde{u}^{{k_l}}_{i,j}\geq 0, l=1,\dots,\sigma(j), h\in\mathcal{H} \label{rate_det}\\
&  \sum_{i=1}^{\tilde{U}_{k,h}}\tilde{u}_{j,h}^{k,i}\underline{R}^k_j \leq z^k_{j,h}W^r_j+(1-x^{k,j^\prime}_j)M, \nonumber \\ 
&\forall k\in\mathcal{K}, j\in V_{gNB},j^\prime \in V_{k,gNB}^\prime, h\in \mathcal{H} \label{rate_det1}
\end{align}
\begin{align}
& z^k_{j,h}W^r_j  \leq \overline{R}^k_j x^{k,j^\prime}_j, \ \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in \mathcal{H} \label{rate_det2}
\end{align}
\begin{align}
% & y_{k,h}^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{\hat{U}_{k,h}} r_k \hat{u}_{k,i,h}^v \quad k =1,...,K, h=1,...,H, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate_det}\\
&  \sum_{k=1}^K z_{j,h}^k \leq 1, \ \forall j\in V_{gNB}, h\in\mathcal{H} \label{cap_ran_det}
\end{align}
{
\begin{align}
% &\sum_{k=1}^K y_{k,h}^v \leq W_v^{tr} \quad h=1,...,H, \forall v\in V_{gNB} \label{cap_ran_det}\\
&  x_j^{k, j^\prime} \geq \mathbbm{1}{\{\sum_{i=1}^{\Tilde{U}_{k,h}} \tilde{u}_{j,h}^{k,i}\geq1\}},\nonumber\\& \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in\mathcal{H} \label{placement_det2}
\end{align}}
\begin{align}
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{\hat{U}_{k,h}} \hat{u}_{k,i,h}^j\geq1\}} \quad k = 1..., K, h=1,...,H, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement_det2}\\
% & x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \quad \forall j\in V, j^\prime \in V^\prime_k, p\in\mathcal{P}_k, e\in E^\prime_k, k\in \mathcal{K}\nonumber \\
& z^k_{j,h} \in [0,1], \eta_{p,h}, \eta_{p,h}^{k,e^\prime}\geq 0, \ \forall k\in \mathcal{K}, j\in V_{gNB}, h\in\mathcal{H} \label{DET-domain_det}
% \end{gather*}
\end{align}
% \end{strip}
We refer to the above problem as $\emph{DET-SMNS}(\mathcal{H})$. The first term in the objective function \eqref{obj_det} is the same as the first term of the objective function \eqref{SMIP:obj}. The second term is the weighted average of the second stage objective function over the $H$ realized samples of the random variables $\chi_k$, $u^k_{i,j}$ and $U_k$. Constraints \eqref{DET-latency-1}-\eqref{DET-domain_det} replace their counterparts. 


It is shown in \cite{shapiro1996simulation} that as the sample size $H$ increases and under certain mild conditions as discussed in \cite{shapiro1996simulation}, the solution to $\emph{DET-SMNS}(\mathcal{H})$ converges to that of the original \emph{SMNS} problem. In the next section, we present a practical algorithm for the resource provisioning of network slicing incorporating the \emph{DET-SMNS} model. 


==> IEEE NetSoft 2023 (1)/model.tex <==
\section{System Model}
\label{sec:sys}



\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4888\textwidth]{figures/E2ENS.png}
    \caption{E2E resource provisioning for multiple NSs}
    \label{fig:E2ENS}
\end{figure}



% We consider the resource provisioning problem of mobile \emph{network slicing} across RAN and CN components. In this section, the network and slice models are presented. 


% We consider the The 5G NS resource allocation problem has two domains, the radio and the core (transport) network resource allocations. While these two problems can be solved separately, a joint approach is more sensible considering the uncertainty about demand points locations. However, obtaining the optimal decision which minimizes the overall cost is not trivial in this case. We propose a two-stage stochastic optimization framework to tackle this problem. In the following, the network and slice models are presented and then the proposed problem formulation is detailed.
\subsection{Substrate Network Model}
We consider a mobile network infrastructure (a.k.a. substrate network) that is comprised of next-generation nodeBs (gNBs) and CN nodes implementing 5GC components. In a mobile network empowered by NFV and SDN, the substrate nodes are general-purpose servers that can host various VNFs. Fig.~\ref{fig:E2ENS} illustrates such an infrastructure. Let $G=(V,E)$ denote the substrate network graph, where $V$ represents the set of substrate nodes and $E$ denotes the set of infrastructure links. We assume that $V = V_{gNB} \cup V_{-gNB}$ where $V_{gNB}$ and $V_{-gNB}$ are the substrate gNB and non-gNB nodes, respectively. Each gNB is characterized by its maximum supported traffic that is computed based on its available resources, or physical resource blocks (PRBs), and antenna configuration. Non-gNB nodes are general-purpose servers providing essential capabilities for running core VNFs. A substrate node is characterized by its residual CPU, storage, and RAM resources. The vector $W_j = (W^{CPU}_j, W^{STO}_j, W^{RAM}_j)$ represents the residual capacity of the substrate node $j\in V$, where we define the set of resources as $\mathcal{T} = \{CPU, STO, RAM\}$. 

Similar to the RAN slicing model considered by \cite{papa2021user}, we assume that the gNB $j\in V_{gNB}$ has $W^{r}_j$ available PRBs that can be allocated to the users of different slices. Furthermore, we assume that $E = E_{FH} \cup E_{BH}$ where $E_{FH}$ and $E_{BH}$ stand for the set of gNB-CN links and the remaining links, respectively. Each substrate link $e\in E$ is characterized by its bandwidth capacity ($W^{BW}_e$) and propagation delay ($\tau^{PRO}_e$). Moreover, let $\mathcal{P}$ denote the set of substrate paths used for traffic routing. Define $\mathcal{P}( i \rightarrow j )$ to be the set of substrate paths between nodes $i$ and $j$. Therefore, $\mathcal{P} = \cup_{i,j\in V, i\neq j} \mathcal{P}( i \rightarrow j )$.
% For the sake of simplicity, we assume that each UE is covered by one gNB and gNBs do not interfere. 
% This can be readily extended to the case with multiple requests per UE by using UE duplication. 
% The SPs meet their customers requested services by dedicating network slices with specified QoS requirements deployed on the substrate network which is owned and managed by InPs. 
Let $\mathcal{U}$ denote the set of UEs distributed across the geographical area under cover. We assume that each UE is served by a gNB according to the nearest association rule, whereby a UE is assigned to the gNB achieving the maximum SNR.
%and $\mathcal{K}$ and the set of network slices
% Therefore, the set of MUs served by gNB $v\in V_{gNB}$ and requesting the service met by slice $k\in \mathcal{K}$ is represented by $U_v^k$.


\subsection{Network Slice Model}
We assume that an NS contains one or multiple SFCs, each comprised of a number of VNFs (e.g. gNB, AFM, UPF, SMF) and virtual links (VLs) between them. The set of NSs is denoted by $\mathcal{K}=\{1,...,K\}$. Let $G^\prime_{k} = (V^\prime_{k}, E^\prime_{k})$ represent the $k$th slice SFC modeled as an undirected graph. 
% Receiving a number of slice/SFC requests, the InP embeds them to the substrate network and allocates sufficient amount of different resources, while making sure that the performance requirements of the SFCs are satisfied. 
We assume $V^\prime_{k} = V^\prime_{k,gNB} \cup V^\prime_{k,-gNB}$ where $V^\prime_{k,gNB}$ and $V^\prime_{k,-gNB}$ correspond to the set of gNBs and non-gNB VNFs of the $k$th slice SFC. Moreover, $E^\prime_{k} =  E^\prime_{k, FH}\cup E^\prime_{k, BH}$ where $E^\prime_{k, FH}$ and $E^\prime_{k, BH}$ denote the fronthaul and backhaul VLs, respectively. We assume that each instance of the SFC corresponding to slice $k$ has QoS requirements expressed as network-level UE throughput and maximum E2E tolerable latency. In order to guarantee the performance requirement of different slices, the network-level performance metric of a slice is translated to cell-level radio resource requirement \cite{8624268}. Let $\underline{R}_j^k$ denote the average required number of PRBs for a UE requesting slice $k\in \mathcal{K}$ covered by gNB $j\in V_{gNB}$. The value of $\underline{R}_j^k$ depends on the overall cell load, antenna configuration, channel condition, modulation and coding scheme (MCS), and slice performance requirements. The details of such a translation mechanism are beyond the scope of this article. We encourage interested readers to refer to \cite{shi2021two} and \cite{oliveira2022mapping} for prospective solutions.
% In accordance with the slice management architecture of \cite{NS}, the overall network slice performance is decomposed into core and RAN domain requirements. Thus, $\underline{R}_j^k$ captures the RAN throughput requirements. Moreover, the value of $\underline{R}_j^k$ is dynamically determined as the condition of different affecting parameters vary. 


We assume that the traffic flow of each $e^\prime \in E^\prime_k$ is routed through substrate paths. Therefore, we represent the set of substrate paths considered for slice $k$ edges by $\mathcal{P}_k$, where $\mathcal{P}_k \subseteq \mathcal{P}$. Let $\mathcal{P}^\prime_k$ denote the set of all paths of $G^\prime_k$. Each path of $G^\prime_k$ corresponds to either CP or UP data flows. For instance, the path gNB-AMF-SMF of a 5G NS is a CP path while gNB-UPF is a UP path. Let $\mathcal{P}^\prime_{k,UP}$ and $\mathcal{P}^\prime_{k,CP}$ denote the set of UP and CP paths in $G^\prime_k$. 
% Hence, $\mathcal{P}^\prime_k = \mathcal{P}^\prime_{k,UP} \cup \mathcal{P}^\prime_{k,CP}$. 
We assume that the QoS requirement of each NS is given as the maximum tolerable UP and CP latencies denoted by $d_{k}^{UP},d_{k}^{CP}$, respectively. Let $\mathcal{U}_k \subseteq \mathcal{U}$ denote the set of UEs requesting slice $k\in\mathcal{K}$. We define $u_j^{k,i}$ to be equal to $1$ if user $i$ of slice $k$ ($i\in \mathcal{U}_k$) is covered by gNB $j\in V_{gNB}$ and $0$, otherwise. 

In order to support the demands of all users requesting an NS, multiple instances of the slice may need to be deployed. Let $I_k$ be the number of instances of slice $k$ deployed to support the load for slice $k$. In addition, each instance of the VNF $j^\prime \in V^\prime_k$ requires CPU, storage, and RAM resources. The required amount of these resources depends on the slice load and the resource-sharing factor which determines how much of the workload of a VNF can be shared among multiple UEs. Let the vector $R_{j^\prime}= (R^{CPU}_{j^\prime}, R^{STO}_{j^\prime}, R^{RAM}_{j^\prime})$ denote the required per-unit amount of CPU, STO and RAM resources for VNF $j^\prime$. Similarly, each VL $e^\prime \in E^\prime_{k}$ is characterized by its per-unit bandwidth requirement $R^{BW}_{e^\prime}$ to meet the demand for data transmission between the two end-points VNFs of $e^\prime$. The per-unit resource requirements must be scaled according to the traffic load and resource-sharing factor. We define $\chi^t_{k,j^\prime}$ to be the scaling factor of resource $\nu$, $\nu\in \mathcal{T}$ for VNFs of slice $k$. 


Moreover, $\chi^{BW}_{k,e^\prime}$ stands for the BW scaling factor of VLs of slice $k$. 
% Therefore, $\chi^\nu_k$ is proportional to $u_j^{k,i}$ and $I_k$.
The cost of running a VNF on the infrastructure node $j$ is composed of two parts: (i) a fixed cost denoted by $C_j$, (ii) a variable cost that increases linearly with respect to the consumed amount of resources by that VNF. Let $C_j^{CPU}, C_j^{STO} $, and $C_j^{RAM}$ denote the per-unit cost of using the CPU, storage, and memory of node $j$, respectively. The per-unit bandwidth cost of the infrastructure link $e$ is represented by $C_e^{BW}$. 
% We consider an environment where UEs can request different services upon transmitting the RRC message with an NS selection assistance information (NSSAI) according to 3GPP specification \cite{}. 
For the sake of simplicity and without loss of generality, we assume that each UE requests at most one slice. A summary of the notations used in this paper is provided in Table \ref{chapter2:parameters}.

%**** In order to speed up the reconfiguration process and minimize VNF migrations resulted from users mobility and change of covering gNB, we assume that all instances of the core VNFs for a NS are embedded on one substrate node in contrast to the virtual gNBs that are essentially placed on different substrate gNBs as required. 

\begin{table}[t]
\centering
\caption{System Model Parameters}
\begin{center}
\scalebox{0.93}{
\begin{tabular}{c|c}
\hline
\hline
Network Parameters & Description\\
\hline
$G = (V, E)$ & Substrate network graph\\
$V_{gNB}, V_{-gNB}$ & Set of substrate gNB and non-gNB nodes\\
$E_{FH}, E_{BH}$ & Set of fronthaul and backhaul links\\
$\mathcal{P}_k$ & Set of substrate paths considered for slice $k$\\
$W_{j}^{r}$ & Available spectrum of gNB $j$\\
$\mathcal{U}_k, U_k$ & Set and number of users of slice $k$\\
$W_j^{CPU,STO,RAM}$ & CPU, Storage and RAM capacities of node $j$\\
$W_e^{BW}$ & BW capacity of the substrate link $e$\\
\hline
\hline
Slice Parameters & Description\\
\hline
$\mathcal{K}, K$ & Set and number of requested slices\\
$G^\prime_{k} = (V_{k}^\prime, E_{k}^\prime)$& The $k$th slice SFC graph\\
$V^\prime_{k,gNB}, V^\prime_{k,-gNB}$ & Set of virtual RAN and core VNFs\\
$E_{k, FH}^\prime, E_{k, BH}^\prime$ & Set of fronthaul and backhaul virtual links\\
$\mathcal{P}^\prime_k$ & Set of slice $k$ E2E paths\\
$\overline{R}_j^k$ & Slice $k$ maximum allowed radio resource in gNB $j$\\
$\underline{R}_j^k$ & Slice $k$ radio resource requirement in gNB $j$\\
$R_{j^\prime}^{CPU, STO, RAM}$ & CPU, Storage and RAM requirements of the VNF $j^{\prime}$\\
$R_{e^\prime}^{BW}$ & BW requirement of the virtual link $e^\prime$\\
$d_{k}^{UP}, d_{k}^{CP}$ & UP and CP latency requirement of slice $k$\\
\hline
\hline
\end{tabular}}
\end{center}
\label{chapter2:parameters}
\end{table}

% \begin{itemize}
% % \item $I_k$: number of virtual gNBs supported by slice $k$ core (not a random variable)
% \item $\chi_k$: scaling factor of BW, compute and storage resources for slice $k$
% \end{itemize}




==> IEEE NetSoft 2023 (1)/prelim.tex <==
\section{Stochastic Programming}
\label{sec:prelim}
In this section, we provide a brief overview of stochastic programming \cite{book}. \textit{Stochastic linear programs} (SLP) are linear programs where some data are uncertain, represented as random variables with given probability measures. The values of these random variables are only known after a random experiment. SLP's optimization decision variables are divided into two groups: first-stage variables, determined before the experiment, and second-stage variables, determined after the experiment results are known.
% The value of the random variables are known only after a random experiment. Hence, the set of optimization decision variables in SLP are divided into two groups: (i) first-stage decision variables, (ii) second-stage decision variables. While the first-stage variables are determined before the random experiment, the second-stage decisions are taken after the random experiment becomes known. 
Let $\boldsymbol{x} \in \mathbb{R}^{n_1\times 1}$ denote the vector of first-stage optimization variables. Define the random variable corresponding to the unknown data as $\boldsymbol{\xi}=\boldsymbol{\xi}(\omega)$ with $\omega\in \Omega$ representing a random event. The vector of second-stage decision variables is denoted by $\boldsymbol{y}(\omega,\boldsymbol{x})$. We assume that the probability distribution $\mathcal{F}$ on $\Omega$ is known in the first stage. The classical two-stage SLP with \textit{fixed recourse} is formulated as follows:
\begin{align}
    & minimize \quad \boldsymbol{c}^T \boldsymbol{x} + \mathbb{E}_{\mathcal{F}}[min\ \boldsymbol{q}(\omega)^T \boldsymbol{y}(\omega,\boldsymbol{x})] \label{SLP-obj}\\
    & s.t. \quad A\boldsymbol{x} = \boldsymbol{b}\label{SLP-c1}\\
    & T(\omega)\boldsymbol{x} + W \boldsymbol{y}(\omega,\boldsymbol{x}) = \boldsymbol{h}(\omega)\label{SLP-c2}\\
    & \boldsymbol{x},\boldsymbol{y}(\omega,\boldsymbol{x}) \geq \boldsymbol{0} \label{SLP-c3}.
\end{align}
where $\boldsymbol{c}\in \mathbb{R}^{n_1\time 1}, \boldsymbol{b}\in \mathbb{R}^{m_1\times 1}, A\in \mathbb{R}^{m_1\times n_1}$. The objective function \eqref{SLP-obj} consists of the deterministic term $\boldsymbol{c}^T \boldsymbol{x}$ and the expectation of the term $\boldsymbol{q}(\omega)^T \boldsymbol{y}(\omega,\boldsymbol{x})$ over all realizations of the random event $\omega$. Note that once the random event $\omega$ is realized, $T(\omega) \in \mathbb{R}^{m_2\times n_2}, \boldsymbol{h}(\omega) \in \mathbb{R}^{m_2\times 1}$, and $\boldsymbol{q}(\omega)\in \mathbb{R}^{n_2\times 1}$ become known. In particular $\boldsymbol{\xi}(\omega) = (\boldsymbol{q}(\omega), \boldsymbol{h}(\omega), T_1(\omega),\dots,T_{m_2}(\omega))$ represents the random data vector where $T_1(\omega),\dots,T_{m_2}(\omega)$ are the rows of $T(\omega)$. For a given $\omega$, let $Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))$ denote the value of the second-stage problem, defined as:
\begin{align}
    & Q(\boldsymbol{x},\boldsymbol{\xi}(\omega)) = min_{\boldsymbol{y}\geq 0} \{\boldsymbol{q}(\omega)^T \boldsymbol{y} | W\boldsymbol{y} = \boldsymbol{h}(\omega)-T(\omega)\boldsymbol{x}\} \label{2-stage-value}
\end{align}
Moreover, the expected value of the second-stage objective value is defined as:
\begin{align}
    & \mathcal{Q}(\boldsymbol{x}) = \mathbb{E}_{\mathcal{F}}[Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))] \label{2-stage-expected-value}
\end{align}
Then, the \textit{deterministic equivalent program} (DEP) corresponding to \eqref{SLP-obj}-\eqref{SLP-c3} is defined as:
\begin{align}
    & min \quad \boldsymbol{c}^T \boldsymbol{x} + \mathcal{Q}(\boldsymbol{x}) \label{DEP-obj}\\
    & s.t. \quad A\boldsymbol{x} = \boldsymbol{b} \label{DEP-c1}\\
    & \boldsymbol{x} \geq \boldsymbol{0} \label{DEP-c2}
\end{align}
The DEP formulation illustrates the major difference between a deterministic linear program and a SLP. Given $\mathcal{Q}(\boldsymbol{x})$, a SLP is an ordinary nonlinear program due to the nonlinearity of $\mathcal{Q}(\boldsymbol{x})$. On the other hand, the computation of $\mathcal{Q}(\boldsymbol{x})$ requires the evaluation of $Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))$ for all $\boldsymbol{x}$ and $\omega$ which is not possible in practice. The problem becomes even more challenging considering the first-stage or second-stage variables to be integers, e.g. $\boldsymbol{x}\in \mathbb{Z}^{n_1}_+$, $\boldsymbol{y}\in \mathbb{Z}^{n_2}_+$. In the next section, we first present our system model for the \emph{network slicing} problem with demand uncertainties followed by our proposed formulation which is based on two-stage stochastic mixed-integer programming. 

==> IEEE NetSoft 2023 (1)/related.tex <==
\section{Related Work}
\label{sec:related}
 To realize \emph{network slicing} in next-generation mobile networks, different required mechanisms including resource provisioning (reservation), slice admission control, resource scheduling, and resource orchestration \cite{hurtado2022deep} have been investigated in the literature for the RAN, TN, CN, or E2E domains.
% that focus on the decision on whether a requested network slice is accepted or rejected and assigning resources to the admitted requests. 
Authors in \cite{9133773} develop an admission control scheme for sliced 5G networks considering inter-slice and intra-slice priorities in order to enhance UEs' QoE and network resource utilization. In \cite{E2E-raof}, the E2E (RAN and CN) resource orchestration of 5G NSs is addressed and a heuristic algorithm for the slice placement problem with the objective of minimizing the number of VNF migrations in the network while optimizing network utilization and satisfying QoS is proposed. 

Authors in \cite{xiang2019joint} study the resource allocation problem of 5G networks leveraging both \emph{network slicing} and mobile edge computing (MEC). They propose an optimization problem with the objective of minimizing the total latency of transmitting, outsourcing and processing user traffic, under the constraint of tolerable latency. In \cite{Tok}, an auction-based model for the joint resource and revenue optimization of RAN and CN NS segments. In all of the aforementioned works, it is assumed that the demand for different slices is known in advance which is an unrealistic assumption. 
% However, the actual distribution of mobile users does not have any effect on the resource allocation strategy and therefore it is not clear how the promised RAN requirement is satisfied in practice. 


In practice, the task of accurately estimating future traffic behavior is very challenging \cite{alliance20155g}. To alleviate this problem, authors in \cite{gholamipour2021online} propose a solution for the joint online admission control and resource allocation problem of \emph{network slicing} using the $\Gamma$-Robustness concept to consider the uncertainty in computation and communication demands. The main drawback of this method is that they only consider the CN slicing problem and ignore the correlation between the demands for different slices. Similarly, a robust model is proposed in \cite{baumgartner2018towards} for the NS design problem under demand uncertainty. In this work, the authors consider both uncorrelated and correlated traffic case which resembles the spatial demand correlations, but they only study the CN design problem. Moreover, they do not consider delay constraints and the differentiation between different slices based on delay requirements. 

% \subsection{Network slicing in RAN or TN or CN}

% \subsection{E2E network slicing}


% Authors in \cite{Tok} proposed an auction-based model for both mobile access and core network to optimize the resources and revenue. However, the actual distribution of mobile users does not have any effect on the resource allocation strategy and therefore it is not clear how the promised RAN requirement is satisfied in practice.
% In \cite{traffic-slice}, a coalitional game was proposed to find the optimal number of slices of 4G or 5G networks to meet the network traffic.
% Authors in \cite{gamma-robust} propose an ILP for the joint optimization of admission control and resource allocation in network slicing, where the uncertainty in computation and communication demands are modeled as stochastic variables with uniform distributions. The stochastic variables are then converted to deterministic ones considering the nominal demand values and their maximum deviations. However, 

%********************************8
% \subsection{Network Slicing under demand uncertainty}
% Authors in \cite{robustNS} propose an optimization framework to handle traffic uncertainties using robust optimization.\cite{wen2018robustness}

% In \ref{reddy2016robust}, a novel optimization
% model based on the concept of ��-robustness to deal with
% uncertainty in the trac demand is proposed. e ��-robust
% optimization is formulated as a MILP. A modied MIP-based
% variable neighborhood search (VNS) heuristic is provided to
% enhance the model’s scalability.



==> IEEE NetSoft 2023 (1)/solution.tex <==
\section{Proposed Solution}
\label{sec:solution}
\subsection{Deterministic Equivalent Reformulation and Sample Average Approximation (SAA)}
In this section, we introduce the deterministic reformulation of the modeled \textbf{SMIP} and then propose a solution based on the sample average approximation (SAA). The SAA method is an approach for solving stochastic optimization problems by using Monte Carlo simulation. Suppose that $H$ realization of the random variables $\chi_k$ and $u_{i,j}^k$, $U_k$ are available denoted by $\hat{\chi}_{k,h}$, $\hat{u}_{i,j,h}^k$,$\hat{U}_{k,h}$, $h = 1,...,H$. For each realization, we have a separate second-stage variable $z_{j,h}^k$. We convert \textbf{SMIP} to its sampled deterministic equivalent problem, defined as follows:
% \begin{strip}
\begin{align}
% \begin{gather*}
% &{minimize} \quad \medmath{\sum_{k=1}^{K} \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) +\phi_3 \sum_{h=1}^H p_h \mathcal{C}_2(\boldsymbol{z}_h)}
% \label{obj_det} \\
&{minimize} \quad \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) +\eta \sum_{h=1}^H \frac{1}{H} \mathcal{C}_2(\boldsymbol{z}_h)
\label{obj_det} \\
&{s.t.} \qquad \qquad \qquad \text{C3,C4}, \text{C6,C7} \label{constraints-moved}\\
& \text{C12}:\ \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \hat{\chi}_{k,h} \leq W_j^{t} \quad \forall t\in \mathcal{T}, j\in V_{}, h\in\mathcal{H} \label{}\\
& \text{C13}:\ \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} \hat{\chi}_{k,h} \leq W_e^{BW} \quad \forall e \in E, h\in\mathcal{H} \label{}\\
% & \text{C14}: \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_k \nonumber\\
% &\forall k\in\mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{path1_det}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{i}^{k,m}-x_{i}^{k,n})\hat{I}_{k,h} \quad k = 1,...,K, h=1,...,H, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path1_det}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path2_det}\\
& \text{C15}: \ z_{j,h}^k W_j^{tr} \geq x^{k,j^\prime}_j\sum_{i = 1}^{\hat{U}_{k,h}} r_k \hat{u}_{i,j,h}^k \nonumber \\ 
&\forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in\mathcal{H} \label{rate_det}\\
% & y_{k,h}^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{\hat{U}_{k,h}} r_k \hat{u}_{k,i,h}^v \quad k =1,...,K, h=1,...,H, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate_det}\\
& \text{C16}: \ \sum_{k=1}^K z_{j,h}^k \leq 1 \quad \forall j\in V_{gNB}, h\in\mathcal{H} \label{cap_ran_det}\\
% &\sum_{k=1}^K y_{k,h}^v \leq W_v^{tr} \quad h=1,...,H, \forall v\in V_{gNB} \label{cap_ran_det}\\
& \text{C17}: \ x_j^{k, j^\prime} = \mathbbm{1}_{\{\sum_{i=1}^{\hat{U}_{k,h}} \hat{u}_{i,j,h}^k\geq1\}}\nonumber\\ &\forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in\mathcal{H} \label{placement_det2}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{\hat{U}_{k,h}} \hat{u}_{k,i,h}^j\geq1\}} \quad k = 1..., K, h=1,...,H, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement_det2}\\
% & x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \quad \forall j\in V, j^\prime \in V^\prime_k, p\in\mathcal{P}_k, e\in E^\prime_k, k\in \mathcal{K}\nonumber \\
& \text{C18}: \quad z^k_{j,h} \in [0,1] \ \forall k\in \mathcal{K}, j\in V_{gNB}, h=1,\dots,H \label{domain_det}
% \end{gather*}
\end{align}
% \end{strip}
We refer to the above problem as \textbf{DET}\_\textbf{MILP}. The first term in the objective function \eqref{obj_det} is same as the first term of the objective function \eqref{SMIP:obj}. The second term is the weighted average of the the second stage objective function over the $H$ realized samples of the random variables $I_k, u^k_{i,j}$ and $U_k$. Constraints C12, C13, C14, C15, C16 replace their counterparts C6, C8, C9, C10, C11 respectively.

In the evaluation section, the performance of this methods is benchmarked against the strategy of providing resources for the worst case scenario, which is the aligned with the way many networks are managed in reality.
%disadvantages: large scale problem, The disadvantage of sampling approaches: some efforts might be wasted on optimizing when distribution approximation is not accurate \cite{book}. 
%Two ways to reduce the problem: Importance sampling and stochastic decomposition.
% \subsection{L-shaped method with implicit enumeration}
% In order to alleviate the complexity arising from large scale second-stage variables and the binary first stage variables, we exploit an integer L-shaped method in this section based on \cite{wo}. 

% \subsection{Adaptive RAN slicing} 


==> IEEE NetSoft 2023 (1)/two-time-scale.tex <==

\section{Two-Timescale Resource Provisioning}
\label{sec:solution}
We propose a two-timescale resource allocation scheme that utilizes the resource provisioning methodology discussed in Sections \ref{sec:sys} and \ref{sec:formulation_thesis}. In this approach, the E2E resource allocation problem of NSs is addressed through two long and short time slots. We assume that the lifecycle of an NS is divided into a number of long time slots (macro-slots) indexed by $T$. During each macro-slot, the demand distribution for NSs is known and fixed. Let $\mathcal{F}^T = \{\mathcal{F}^T_1,\dots,\mathcal{F}^T_K\}$, where $\mathcal{F}_k(.,.):\mathbb{R}^2 \xrightarrow{} [0,1]$ denote the spatial density function of the $k$th slice demand across the considered geographical area in the macro-slot $T$. Given $\mathcal{F}^T$, we solve the resource provisioning problem proposed in Section \ref{sec:DEF}, $\emph{DET-SMNS}(\mathcal{H})$. 


We further divide each macro-slot into $N_T$ short time slots (micro-slots). At each micro-slot $t$, the actual demand is observed that is shown by $\hat{\boldsymbol{\xi}}=(\hat{\mathcal{U}}_k, \hat{u}^{k,i}_{j}, \hat{\chi}^\nu_k, k\in\mathcal{K},i\in \hat{\mathcal{U}}_k, j\in V_{gNB},\nu\in\mathcal{T}\cup\{BW\})$. We define the decision variable $\sigma^k_j, k\in \mathcal{K}, j\in V_{gNB}$ as the fraction of unsupported demand requested for slice $k$ in gNB $j$. Given the observed demand at each micro-slot, and the solution to the first-stage problem ($\boldsymbol{x}, \boldsymbol{y}$), we adjust the RAN resource provisioning decision by solving the following linear program (LP):
\begin{align}
    & {minimize}\quad  \sum_{k\in\mathcal{K}}\sum_{j\in V_{gNB}} \theta (\mathcal{C}_2(\boldsymbol{z})) +  (1-\theta)\sigma^k_j \label{real:obj}
\end{align}
    % & \frac{1}{\sum_{i=1}^{U^o_{k_1}}u^{o,k_1}_{i,j}}z^{k_1}_j = \dots = \frac{1}{\sum_{i=1}^{U^o_{k_{\sigma(j)}}}u^{o,k_{\sigma(j)}}_{i,j}}z^{k_{\sigma(j)}}_j \nonumber\\
    % & \forall j\in V_{gNB}, k_l \in \mathcal{K}, \sum_{i=1}^{U^o_{{k_l}}}u^{o,{k_l}}_{i,j}\geq 0, l=1,\dots,\sigma(j) 
\begin{align}
    & (1-\sigma^k_j)(\sum_{i=1}^{\hat{{U}}_k} \hat{u}^{k,i}_{j}) \underline{R}^k_j \leq z^k_j W^r_j + (1-x^{k,j^{\prime}}_{j})M, \nonumber\\ 
    &\forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{real:one}
\end{align}
\begin{align}
    & \frac{\sum_{j\in V_{gNB}}(1-\sigma^k_j) \sum_{i=1}^{\hat{U}_k}\hat{u}^{k,i}_j}{\hat{U}_k}\hat{\chi}^\nu_k \leq \chi^\nu_{k,prov}, \nonumber\\ 
    &\forall k\in\mathcal{K}, \nu\in \mathcal{T}\cup \{BW\} \label{real:two}
\end{align}
\begin{align}
    & z^k_j W^r_j \leq \overline{R}^k_j x^{k,j^\prime}_j, \ \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V^\prime_{k,gNB}\label{real:three}
\end{align}
\begin{align}
    & \sum_{k\in\mathcal{K}}z^k_j\leq 1,\ \forall j \in V_{gNB} \label{real:four}
\end{align}
\begin{align}
    & z^k_j, \sigma_j^k \in [0,1], \ \forall k\in \mathcal{K}, j\in V_{gNB} \label{real:five}
\end{align}
We refer to this LP as the radio network slicing resource allocation, denoted by $\emph{RNSR}(\boldsymbol{x},\boldsymbol{y}, \hat{\boldsymbol{\xi}} )$.

The objective of \eqref{real:obj} minimizes the weighted summation of RAN resource allocation cost and total unsupported traffic. The weight parameter $\theta \in [0,1]$ is used to balance between the two objective terms. Constraint \eqref{real:one} ensures that the radio resource reservation for an NS is greater than the supported traffic on each gNB. $M$ is a big positive real value used for the big-M method, enforcing constraint \eqref{real:one} for a tuple $(j', k, j)$ only if $x^{k,j'}_j = 1$, i.e. a RAN VNF of slice $k$ is instantiated on gNB $j$. Constraint \eqref{real:two} guarantees the availability of core network resources to support the admitted traffic of each slice. The slice isolation constraint is enforced by \eqref{real:three}. Constraint \eqref{real:four} ensures the capacity constraint for each gNB, and the domain constraints are expressed by \eqref{real:five}. Algorithm \ref{algo}  illustrates our proposed two-timescale resource provisioning scheme.



% Figure \ref{twotime} illustrates our proposed two-timescale resource allocation scheme. Given the demand distribution $\mathcal{F}^T$ for each long time slot, we solve an instance of $\textbf{DET}\_\textbf{SMNS}(\mathcal{H})$ that provides the resource provisioning solution for the core network. Given the core network slicing solution and a realization of the slices' demand points at each short time slot, the $\textbf{SMNS}(\boldsymbol{x},\boldsymbol{y}, \hat{\boldsymbol{\xi})$ problem is solved to obtain the E2E resource allocation solution. The instantaneous demand for different network slices at each short time slot is used to scale down/up the core network slices if needed.  
\begin{algorithm}[t]
 \caption{Two-timescale Resource Provisioning}
 \label{algo}
 \begin{algorithmic}[1]
 \Statex \textbf{Input: } $G$, $G^\prime_k, \mathcal{U}_k, k\in\mathcal{K}$
 \Statex \textbf{Output: } $\boldsymbol{x}$, $\boldsymbol{y}$, $\boldsymbol{z}, \sigma$
 \For{$T=1,\dots$}
 \State Find $\mathcal{F}^T$ using historical demand distribution data.
 \State Take $H$ sample of $\mathcal{F}^T$, denoted by the set $\mathcal{H}$.
 \State $(\boldsymbol{x, y}) \xleftarrow{}$ Solve $\emph{DET-SMNS}(\mathcal{H})$.
 \For{$t=1,\dots,N_T$}
 \State Observe $\hat{\boldsymbol{\xi}}$.
 \State $(\boldsymbol{z, \sigma})\xleftarrow{}$ Solve $\emph{RNSR}(\boldsymbol{x},\boldsymbol{y},\hat{\boldsymbol{\xi}})$
 \EndFor
 \EndFor
 \end{algorithmic} 
 \end{algorithm}
 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/twotime-2.png}
%     \caption{Two-Timescale Resource Provisioning Scheme}
%     \label{twotime}
% \end{figure}
% \subsection{L-shaped method with implicit enumeration}

% \section{Decomposition Algorithm}
% In this section, we propose an algorithm to solve the proposed \textbf{DET}\_\textbf{SNSR}  problem efficiently. Using the Benders decomposition method, we decompose problem \textbf{DET}\_\textbf{SNSR} into a master problem and $H$ subproblems. In this approach, the objective value of the second-stage problem is approximated iteratively by solving the subproblems that return feasibility and optimality cuts. This process continues until no more cuts are found or a given optimality gap is achieved. The Benders master problem is:
% \begin{align}
%     & MP(\mathcal{H}):\quad minimize \quad \mathcal{C}_1(\boldsymbol{x}, \boldsymbol{y}) + \eta \sum_{h=1}^H \frac{1}{H} \sigma_h \\
%     & s.t. \quad \eqref{SIMP:non-gNB-map1} - \eqref{SMIP:dom1}\\
%     & (\sigma_h, \boldsymbol{x}, \boldsymbol{y}) \in \Sigma_h, \ h\in \mathcal{H}
% \end{align}
% where $\Sigma_h$ is ...
% For a given scenario $h$ and first-stage solution $(\hat{\boldsymbol{x}}, \hat{\boldsymbol{y}})$, the subproblems corresponding to each scenario are:
% \begin{align}
%     & SP(\hat{\boldsymbol{x}},\hat{\boldsymbol{y}}, h): \quad minimize \quad \mathcal{C}_2(\boldsymbol{z})\\
%     % & \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} \hat{x}_{j}^{k,j^\prime} R_{j^\prime}^{t} \tilde{\chi}_{k,h} \leq W_j^{t},\ \forall t\in \mathcal{T}, j\in V_{}, h\in\mathcal{H} \label{Dec-cap1}\\
%     % & \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} \hat{y}^{k,e^\prime}_p R^{BW}_{e^\prime} \tilde{\chi}_{k,h} \leq W_e^{BW},\ \forall e \in E, h\in\mathcal{H} \label{Dec-cap2}\\
%     & \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} \hat{x}_{j}^{k,j^\prime} R_{j^\prime}^{t} \tilde{\chi}_{k,h} \leq W_j^{t},\ \forall t\in \mathcal{T}, j\in V_{}\\
%     & \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} \hat{y}^{k,e^\prime}_p R^{BW}_{e^\prime} \tilde{\chi}_{k,h} \leq W_e^{BW} ,\ \forall e \in E \\
%     & \sum_{i=1}^{\tilde{U}_{k,h}}\tilde{u}_{i,j,h}^k\underline{R}^k_j \leq z^k_{j,h}W^r_j+(1-\hat{x}^{k,j^\prime}_j)M, \ \forall k\in\mathcal{K}, j\in V_{gNB},j^\prime \in V_{k,gNB}^\prime\\
%     & z^k_{j,h}W^r_j  \leq \overline{R}^k_j \hat{x}^{k,j^\prime}_j, \ \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime\\
%     & \sum_{k=1}^K z_{j,h}^k \leq 1,\ \forall j\in V_{gNB}\\
%     & 
% \end{align}

% \begin{figure}
%     \centering
% \includegraphics[width=0.45\textwidth]{figures/pdf_example_2.jpg}
%     \caption{An Example of a Slice Demand Probability Distribution}
%     \label{fig:kde_example}
% \end{figure} 








==> evaluation.tex <==
\section{Performance Evaluation}
\label{sec:evaluation}
We have implemented an evaluation environment in Java, including a network slice generator and a cellular network topology generator. We use ILOG CPLEX solver interfaced with Java for embedding and solving MILP/LP models. A rectangle area of dimension $1000(m)\times1000(m)$ is considered in all the results of this section. Figure \eqref{fig:top} shows the general structure of the substrate network topology used in the experiments. It consists of 40 gNBs and 7 core nodes. The gNBs are placed randomly and a voronoi tessellation is constructed using euclidean distance to assign users to gNBs. We assume to have three different network slices, namely eMBB, URLLC and mMTC with data rate requirements showed in Tables \eqref{Slices}. All NSs have graphical architecture of Figure (1). Users are distributed according to a spatial poisson point process with mean $\lambda = 50$. The requests by users for each slice is randomly chosen. Without loss of generality, we assume that each user can request at most one NS. This is a valid assumption because if any user in the network requests for more than one slices, we can substitute it with two users each requesting one NS. 
\begin{table}[ht]
\centering
\begin{center}
\scalebox{0.9}{
\begin{tabular}{|c|c|}
\hline
\hline
Slice type & Data rate & Latency\\
\hline
eMBB & 100Mbps &\\
ULRRC & 10Mbps &\\
mMTC & 1 Mbps &\\
\hline
\hline
\end{tabular}}
\end{center}
\caption{Data rate requirements of different type of slices}
\label{Slices}
\end{table}
The performance of the SAA method is compared with a solution based the worst case scenario (\textbf{Worst}\_\textbf{MILP}) that provisions resources to serve an overloaded network with $30\%$ more network load than normal. In this case, a smaller MILP with $H=10$ is solved to find the optimal resource allocation decision. These kinds of resource overprovisioning is very close to the way todays' networks are managed in order to avoid severe service degradation in the time of pick traffic. 
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/topology.png}
  \caption{Network topology}
    \label{fig:top}
\end{figure} 
Figure \eqref{fig:time} compares the solver run time of \textbf{DET}\_\textbf{MILP} with \textbf{Worst}\_\textbf{MILP} for different number of samples. The results are averaged on $5$ generated scenarios of users distribution for each sample size. As expected, the solver run time of \textbf{DET}\_\textbf{MILP} increases when more samples are considered. Figure \eqref{fig:box} illustrates the solver run time profile for the two methods where $H=50$ samples are considered in \textbf{DET}\_\textbf{MILP} and the results are collected for 10 runs.

Figure \eqref{fig:sup} depicts the supported traffic as the number of considered samples changes. In this experiment, after the resource allocation problems \textbf{DET}\_\textbf{MILP} and \textbf{Worst}\_\textbf{MILP} are solved, a new network instance is generated and the supported traffic is computed. It can be observed that as the number of samples increases, SAA can better provision resources and the total network supported traffic can come very close to the case that an artificial overloaded network is considered for resource allocation as in \textbf{Worst}\_\textbf{MILP}. An interesting metric that can be compared in this regard is the amount of idle resources for the two methods in different network loads. Finally, the deployment cost of \textbf{Worst}\_\textbf{MILP} and \textbf{DET}\_\textbf{MILP} is compared in Figure \eqref{fig:cost} when $H=50$, which confirms that since the former allocates more resources than needed, its deployment cost increases (many allocated resources remain idle). Last but not least, it should be noted that although \textbf{Worst}\_\textbf{MILP} performs worst than \textbf{DET}\_\textbf{MILP} in terms of cost, it does not require as much as prior knowledge required by \textbf{DET}\_\textbf{MILP}, therefore, is it less sensitive to misinformation (when the actual data distribution is different from the considered distribution). Moreover, in these methods some efforts might be wasted optimizing when distribution approximation and sampling is not accurate. A future approach to reduce this bias on prior knowledge could be exploring sampling methods other than Crude Monte Carlo. Stochastic decomposition and importance sampling can be used along with the L-shaped method in order to alleviate this problem.
\begin{figure*}[t]
\begin{center}
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/time.png}
\caption{Average solver run time of \textbf{DET}\_\textbf{MILP} vs. \textbf{Worst}\_\textbf{MILP}}  
\label{fig:time}
\end{minipage} 
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/box_time.png}
  \caption{The profile of solver run time ($H = 50$ for \textbf{DET}\_\textbf{MILP})}
    \label{fig:box}
\end{minipage}\\
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/sup.png}
  \caption{Comparison of supported traffic, \textbf{DET}\_\textbf{MILP} vs. \textbf{Worst}\_\textbf{MILP}}
    \label{fig:sup}
\end{minipage}
\begin{minipage}[h]{0.45\textwidth}
\includegraphics[width=0.8\textwidth]{figures/cost.png}
  \caption{Comparison of deployment cost, \textbf{DET}\_\textbf{MILP} vs. \textbf{Worst}\_\textbf{MILP}}
    \label{fig:cost}
\end{minipage}
\end{center}
\end{figure*}

==> formulation.tex <==
\section{System Model and Problem Formulation}
Time intervals...
A summary of the parameters is given in Table \ref{parameters}.
\label{sec:sys}
% We consider the The 5G NS resource allocation problem has two domains, the radio and the core (transport) network resource allocations. While these two problems can be solved separately, a joint approach is more sensible considering the uncertainty about demand points locations. However, obtaining the optimal decision which minimizes the overall cost is not trivial in this case. We propose a two-stage stochastic optimization framework to tackle this problem. In the following, the network and slice models are presented and then the proposed problem formulation is detailed.
\subsection{Infrastructure Network model}
Let the infrastructure network (substrate) be represented as a directed graph $G = (V, E)$, where $V$ is the set of infrastructure nodes and $E$ denotes the set of infrastructure links. The set of infrastructure network nodes consists of two type of nodes, gNB and non-gNB. Thus, $V = V_{gNB} \cup V_{-gNB}$ where $V_{gNB}$ and $V_{-gNB}$ correspond to the set of substrate gNB and non-gNB node, respectively. Each gNB is characterized by its maximum supported traffic which is computed based on its available bandwidth (physical resource blocks or PRBs) and MIMO antenna configuration. Non-gNBs are general-purpose servers providing essential capabilities for running core network functions (NFs) and could data centers. A substrate node is characterized by its available CPU, storage and RAM resources. We define the set of node resources as $\mathcal{T} = \{CPU, STO, RAM\}$. Let the vector $W_j = (W^{CPU}_j, W^{STO}_j, W^{RAM}_j)$ represent the available capacity of the substrate node $j$. These amounts correspond to the initial capacity of the node reduced by the amount allocated to previously accepted concurrent requests. Moreover, the cost of each infrastructure node $j$ being used by a VNF consists of two parts: (i) a fixed part $C_j$ paid for each VNF deployed on node $j$, (ii) a variable part associated to the per-unit usage of each resource which depends linearly on the amount of the resource consumed by a VNF. The per-unit variable cost corresponding to CPU, storage and memory of node $j$ are denoted by $C_j^{CPU}, C_j^{STO} $ and $C_j^{RAM}$. 

We assume that each gNB offers  wireless resources to MUs. The maximum traffic supported by gNB $j\in V_{gNB}$ is shown by $W^{tr}_j$. Furthermore, the set of infrastructure link $E = E_{FH} \cup E_{BH}$ where $E_{FH}$ and $E_{BH}$ stand for the links between gNB nodes and the core network and the remaining link, respectively. Each substrate link $e\in E$ has a bandwidth capacity and propagation delay denoted by $W^{BW}_e$ and $\tau^{PRO}_e$ in respective order. Moreover, a per-unit bandwidth cost is associated to the infrastructure link $e$ denoted by $C_e^{BW}$. In order to meet the traffic transmission between two VNFs of a network slice, we consider a set of substrate paths denoted by $\mathcal{P}$. 
% For the sake of simplicity, we assume that each UE is covered by one gNB and gNBs do not interfere. 

We consider an environment in which MUs submit their request for different services to SPs. For the sake of simplicity, we assume that each user requests at most one service. This can be readily extended to the case of multiple requests from a user by duplicating MUs that have multiple service requests. Each service is realized through network slices managed by SPs. The SPs meet their customers requested services by dedicating network slices with specified QoS requirements deployed on the substrate network which is owned and managed by InPs. Let $U$ denote the set of MUs distributed across the considered geographical area. We assume that each MU is served by a gNB according to the nearest association rule. 

For a user 
%and $\mathcal{K}$ and the set of network slices
% Therefore, the set of MUs served by gNB $v\in V_{gNB}$ and requesting the service met by slice $k\in \mathcal{K}$ is represented by $U_v^k$.

\subsection{Network Slice Model}
In this section, we present the network slice model. We assume that a slice request is modeled as one or multiple service function chains (SFCs), each consisting of a number of VNFs (e.g. gNB, AFM, UPF, SMF) and virtual links (VLs) between them. The set of system network slices is represented by $\mathcal{K}=\{1,...,K\}$. Let the directed graph $G^\prime_{k} = (V^\prime_{k}, E^\prime_{k})$ describe the $k$th slice' SFCs. Similarly to the substrate network, we assume that the nodes of slice $k$ consist of two types of nodes, gNB and non-gNB. Therefore, $V^\prime_{k} = V^\prime_{k,gNB} \cup V^\prime_{k,-gNB}$ where $V^\prime_{k,gNB}$ and $V^\prime_{k,-gNB}$ correspond to the set of gNBs and non-gNB functions of slice $k$. Moreover, $E^\prime_{k} =  E^\prime_{k, FH}\cup E^\prime_{k, BH}$ where $E^\prime_{k, FH}$ and $E^\prime_{k, BH}$ denote the fronthaul and backhaul VLs, respectively. 
We assume that each instance of the SFC corresponding to slice $k$ has QoS requirements expressed as gNB's spectrum $r_k$ and maximum E2E acceptable latency $d_k$. In addition, each VNF instance of the node $j^\prime$ in slice $k$ requires the CPU, storage and RAM resources, represented by the vector $R_{j^\prime}= (R^{CPU}_{j^\prime}, R^{STO}_{j^\prime}, R^{RAM}_{j^\prime})$. Similarly, each VL $e^\prime \in E^\prime_{k}$ is characterized by the bandwidth requirement of $R^{BW}_{e^\prime}$ to meet the demand for data transmission between the two end-pints (VNFs) of $e^\prime$. We assume that the traffic flow of each $e^\prime \in E^\prime_k$ is routed through substrate paths. Therefore, we represent the set of substrate paths considered for slice $k$ edges by $\mathcal{P}_k$, where $\mathcal{P}_k \subseteq \mathcal{P}$.

In order to satisfy the demands of all users requesting a network slice, multiple instances of that slice may be required to be deployed. We define the parameter $u_v^{k,i}$ which is equal to $1$ if user $i$ of slice $k$ is covered by gNB $v$ and $0$ otherwise. Moreover, the parameter $I_k$ indicates the number of instances of slice $k$ needed to be deployed in order to support the demand for slice $k$. Due to the mobility of the MUs and their varying demands, the true values of $u_v^{k,i}$ and $I_k$ are not known. However, given the historical data on the demand and mobility patterns of MUs, the SP and InP are capable of estimating the statistical characteristics of $u_v^{k,i}$ and $I_k$. We assume that at each time instance, the spatial distribution of demand points for different network slices are given, represented by $\mathcal{F}_1,\dots,\mathcal{F}_k, k\in \mathcal{K}$. Hence, $u_v^{k,i}$ and $I_k$ become random variables with known distributions. Define $\mathcal{F} = \{\mathcal{F}_1,\dots,\mathcal{F}_k\}, k\in \mathcal{K}$.
%**** In order to speed up the reconfiguration process and minimize VNF migrations resulted from users mobility and change of covering gNB, we assume that all instances of the core VNFs for a NS are embedded on one substrate node in contrast to the virtual gNBs that are essentially placed on different substrate gNBs as required. 
\begin{figure}[!t]
\centering
\includegraphics[width=0.35\textwidth]{figures/slice.png}
  \caption{A network slice example}
    \label{fig:slice}
\end{figure}
\begin{table*}[t]
\centering
\begin{center}
\scalebox{1}{
\begin{tabular}{c|c}
\hline
\hline
Network Parameters & Description\\
\hline
$G = (V, E)$ & The substrate network graph\\
$V_{gNB}, V_{core}$ & The set of substrate RAN and core nodes\\
$E_{FH}, E_{BH}$ & The set of fronthaul and backhaul links\\
$W_{v}^{tr}$ & maximum traffic rate supported by gNB $v$\\
$U^k$ & Number of users of slice $k$ in the network\\
$W_j^{CPU,STO,RAM}$ & The amount of CPU, Storage, and RAM capacities of the substrate node $j$\\
$W_e^{CAP}$ & The capacity of the substrate link $e$\\
\hline
\hline
Slice Parameters & Description\\
\hline
$K$ & Number of requested slices\\
$G^k_{slc} = (V_{slc}^k, E_{slc}^k)$& The $k$th slice SFC graph\\
$V^k_{slc,ran}, V^k_{slc,core}$ & the set of virtual RAN and core VNFs\\
$E_{slc, FH}^k, E_{slc, BH}^k$ & The set of fronthaul and backhaul virtual links\\
$r_k$ & slice $k$ rate requirement\\
$R_{j^\prime}^{CPU, STO, RAM}$ & The amount of CPU, Storage and RAM resource requirements of the VNF $j^{\prime}$\\
$R_{e^\prime}^{CAP}$ & The data rate requirement of the virtual link $e^\prime$\\
\hline
\hline
\end{tabular}}
\end{center}
\caption{System model parameters}
\label{parameters}
\end{table*}

\subsection{Problem formulation}
% Figure \ref{fig:architecture} illustrates an example of E2E resource allocation for different slices. 
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/architecture.png}
%   \caption{An example of the E2E slice resource allocation}
%     \label{fig:architecture}
% \end{figure} 
% The problem architecture is illustrated at the bottom of this figure.
%The main consideration is that the problem is solved for a set of gNBs connected to a single gateway acting as an aggregation point. 
Given the substrate network and network slice graphs, we formulate the problem of E2E network slicing under demand uncertainty as a two-stage SMIP, using the following variables:
\begin{itemize}
\item A set of binary variables $\boldsymbol{x}_{k}$ where $x_j^{k,j^\prime}$ is $1$ if the an instance of VNF $j^\prime$ of the $k$th slice is placed at substrate node $j$.
\item A set of binary variables $\boldsymbol{y}_{k}$ where $y_p^{k,e^\prime}$ is 1 if the virtual link $e^\prime$ of the $k$th slice is assigned to substrate path $p$.
\item A set of continuous decision variables $\boldsymbol{z}_k$ where $z_j^k$ represents the fraction of gNB $j$ supported traffic that is allocated to slice $k$.
\end{itemize}
It is important to note that the value of the vector $\boldsymbol{z} = (z_1^1,...,z_{|V_{gNB}|}^1,...,z_1^K,...,z_{|V_{gNB}|}^K)$ represents the RAN slicing policy defined as the fraction of each cell available spectrum that is assigned to each requested slice. For example, in the case of having three network slices, the subsequent RAN slice allocation for a gNB can be $20\%, 50\% $, and $30\%$. Once this spectrum assignment policy is determined, the actual radio resource allocation in terms of the number of PRBs allocated to the users of each slice to fulfill the spectrum requirement is formulated separately. In this regard, different solutions have been proposed in the literature with the goal of minimizing the interference between different mobile virtual network operators \cite{RAN}. 

We model the resource provisioning problem for the requested slices as a two-stage SMIP. We refer to this method as \textbf{SMIP} which is described in the following sections.

\subsubsection{First-stage problem}
The first-stage objective in \textbf{SMIP} is the minimization of the total provisioning cost which consists of node and link deployment costs for all slices. Let $\mathcal{C}_k^{N}$ and $\mathcal{C}_k^{L}$ denote the node and link costs corresponding to slice $k$, respectively. Consequently, we have:
% \begin{strip}
\begin{equation}
    \mathcal{C}_k^N(\boldsymbol{x}_{k}) = \sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}C_j^kx_{j}^{k}+\sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}\sum_{t\in \mathcal{T}}R_{j^\prime}^tC_j^t x_j^{k,j^\prime}
    \label{SMIP:node-cost}
\end{equation}
\begin{equation}
    \mathcal{C}_k^L(\boldsymbol{y}_{k}) = \sum_{p\in\mathcal{P}}\sum_{e\in p}\sum_{e^\prime \in E^\prime_k} R_{e^\prime}^{BW} C_e^k y_{p}^{k, e^\prime}
    \label{SMIP:link-cost}
\end{equation}
% +\phi_2\sum_{e\in E}\sum{e^\prime \in E^\prime_k} z_{e}^{k, e^\prime} C_e^k) +\phi_3\mathbb{E} Q_{x,z}(u)
where
\begin{equation}
  x_{j}^{k} =
    \begin{cases}
      1 & \text{if $\sum_{j^\prime\in V^\prime_{k}}x_j^{k,j^\prime} \geq 0$}\\
      0 & \text{otherwise}
    \end{cases}       
\end{equation}
Hence, the first-stage objective is: \begin{equation}
     \mathcal{C}_1 (\boldsymbol{x},\boldsymbol{y}) = \phi_1\sum_{k\in\mathcal{K}}\mathcal{C}^N_k(\boldsymbol{x}_k)+\phi_2 \sum_{k\in\mathcal{K}}\mathcal{C}^L_k(\boldsymbol{y}_k)
     \label{SMIP:Obj1}
\end{equation}
where $\phi_1$ and $\phi_2$ are constants to balance between the two objective terms of \eqref{SMIP:node-cost} and \eqref{SMIP:link-cost}.
% +\phi_3\mathbb{E} Q_{x,y}(U)

For each infrastructure node and link, we have capacity constraints as follows:
\begin{equation}
    \text{C1}:\ \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} I_k \leq W_j^{t} \quad t\in \mathcal{T}, \forall j\in V_{} \label{SIMP:node-Cap1}
\end{equation}
\begin{equation}
    \text{C2}:\ \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} I_k \leq W_e^{BW} \quad \forall e \in E
    \label{SIMP:link-Cap1}
\end{equation}
Moreover, in a feasible resource provisioning solution, each gNB VNF is placed at one substrate gNB node and each non-gNB VNF runs on a substrate non-gNB node. Thus, the resulting VNFs deployment must guarantee the following constraints:
% \begin{equation}
%     \text{C3}:\ \sum_{j\in V_{gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,gNB}
%     \label{SIMP:gNB-map1} -->removed
% \end{equation}
\begin{equation}
    \text{C3}:\ \sum_{j\in V_{-gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,-gNB}
    \label{SIMP:non-gNB-map1}
\end{equation}
Let $\mathcal{P}^\prime_k$ denote the set of all paths of slice $k \in \mathcal{K}$. The execution latency of VNF $j^\prime \in V^\prime_k$ on the infrastructure node is represented by $\tau^{k,j^\prime}$. Given the edge mapping decision variables $y^{k,e^\prime}_p$, the data transmission latency corresponding to the infrastructure edge $e\in E$ based on its aggregated assigned data demand is computed in equation \eqref{d-edge}.
\begin{equation}
    \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e} \label{d-edge}
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ mapped to the path $p\in \mathcal{P}_k$ is:
\begin{equation}
    \sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ is computed in equation \eqref{d-slice-edge}.
\begin{equation}
    \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \label{d-slice-edge}
\end{equation}
The latency of slice $k$ instances experienced by the MUs of that slice is guaranteed to be lower than the required latency of the slice in constraints \eqref{SIMP:latency-1}.
\begin{align}
    & \text{C4}: \nonumber\\
    & \sum_{e^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \right]\nonumber\\
    & + \sum_{j^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \right]  \leq d_k\quad \forall p^\prime \in \mathcal{P}^{\prime}_k, k\in \mathcal{K} \label{SIMP:latency-1}
\end{align}
Finally, the domain constraints are presented as follows:
\begin{align}
    & \text{C5}: 
    x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \ k\in \mathcal{K}, j\in V, j^\prime \in V^\prime_k, p\in \mathcal{P}_k, e^\prime \in E^\prime_k \label{SMIP:dom1}
\end{align}
% \begin{align}
%&\textbf{s.t} \nonumber \\
%& \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% &\sum_{e\in\delta^+(j)} z_{e}^{k, e^\prime} - \sum_{e\in\delta^-(j)}z_{e}^{k, e^\prime} = 
    %\left\{
    %\begin{array}{@{}ll@{}}
    %1 & if \quad j = destination(e^\prime)\\
    %-1 &  if \quad j = source(e^\prime)\\
    %0 & otherwise\\
    %\end{array}\right. \quad k=1,...,K, \forall j \in V, e^\prime \in E^k_{slc} \label{path}\\
% &\sum_{k=1}^K \sum_{j^\prime\in V_{slc}^k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \leq W_j^{t} \quad t\in \{CPU, STO, RAM\}, \forall j\in V_{} \label{node_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,FH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{FH}\label{link_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,BH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{BH}\label{link_cap2}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{}\label{link_cap1}\\
% &\sum_{j\in V_{core}}x_{j}^{k,j^\prime} = 1 \quad k=1,...,K, \forall j^\prime \in V^k_{slc,core} \label{placement1}\\
% & x_j^{k, j^\prime}\in \{0,1\}, z_{e}^{k,e^\prime} \geq 0  \quad k = 1,...,K, j\in V, j^{\prime}\in V^{k}_{slc}, e\in E, e^\prime \in E^k_{slc} \label{domain1}
% \end{align} 
% \end{strip}

%%second stage
\subsubsection{Second-stage problem} The goal of the second-stage problem is to minimize the total gNB traffic allocated to network slices. 
The second-stage objective is:
\begin{equation}
     \mathcal{C}_2(\boldsymbol{z}) = \sum_{k\in\mathcal{K}}\sum_{j\in V_{gNB}} z^k_{j}
\end{equation}
The flow conservation constraints are guaranteed by equations \eqref{SIMP:flow2-nongNB} and \eqref{SIMP:flow2-gNB}.  
\begin{align}
    & \text{C6}:\ \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_{k} \nonumber\\
    &\qquad\qquad\forall k\in\mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{SIMP:flow2-nongNB}
\end{align}
\begin{align}
    & \text{C7}:\ \sum_{\substack{p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\  j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} - y_{q(j \rightarrow i)}^{k,e^\prime} = x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime} \nonumber \\
    &\qquad\qquad \forall k\in \mathcal{K}, i\in V_{gNB}, e^\prime(i^\prime \rightarrow j^\prime)\in E_{k,FH}^\prime \label{SIMP:flow2-gNB}
\end{align}
The traffic allocated to the users of a slice must be greater than the required traffic of slice k. This constraint is ensured by equations \eqref{SIMP:reqrate}.
\begin{align}
    & \text{C8}:\ z_j^k W_j^{tr} \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\ 
    & \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
\end{align}
% \begin{align}
%     & \text{C8}:\ c k_i (1-BER_i) \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\
%     &\quad \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
% \end{align}
The capacity constraint of gNBs is enforced by equation \eqref{SIMP:gNBcap}. 
% \begin{equation}
%     \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq W_j^{tr} \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
% \end{equation}
\begin{equation}
    % \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
    \text{C9}:\ \sum_{k=1}^K z_{j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
\end{equation}
The gNB placement constraints are enforced by equation \eqref{SIMP:gNBplacement2}.
\begin{equation}
    \text{C10}: \ x_j^{k, j^\prime} = \mathbbm{1}_{\{\sum_{i=1}^{U_k} u_{i,j}^k\geq1\}} \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:gNBplacement2}\\
\end{equation}
The domain constraints of the second-stage problem are:
\begin{align}
    & \text{C11}: \ z^k_j \in [0, 1] \quad \forall k\in \mathcal{K}, j\in V_{gNB},  \label{domain2} 
\end{align}
% Let $Q(\boldsymbol{x},\boldsymbol{y}, U)$ denote the optimal value of the second-stage problem. 
The E2E network slicing problem with demand uncertainties is formulated as a two-stage SMIP presented below:
\begin{align}
    & {minimize} \quad \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) + \eta \ \mathbb{E}_{
    \mathcal{F}} [min \ \mathcal{C}_2 (\boldsymbol{z})] \label{SMIP:obj} \\
    & \qquad \qquad \qquad \text{s.t.}  \qquad \text{C1}-\text{C11} \nonumber
\end{align}
% $Q_{x,z}(u)$ is the optimal value of the second-stage defined as follows:
% \begin{strip}
% \begin{align}
% &\textbf{minimize}
% \quad \sum_{k=1}^{K} (\sum_{v\in V_{gNB}} z_k^v) \label{obj2}\\
% &\textbf{s.t} \nonumber \\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{j}^{k,m}-x_{j}^{k,n})I_{k} \quad k = 1,...,K, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path2}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% & y_k^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{U_k} r_k u_{k,i}^v \quad k =1,...,K, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate}\\
% &\sum_{k=1}^K y_k^v \leq W_v^{tr} \quad \forall v\in V_{gNB} \label{cap_ran}\\
%&\sum_{}z_{e}^{e^\prime , k}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{U_k} u_{i,k}^j\geq1\}} \quad k = 1..., K, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement2}\\
% & y_k^v \in [0, W_v^{tr}], \quad k = 1..., K, \forall  v\in V_{gNB},  \label{domain2}
% \end{align}
% \end{strip}
The objective \eqref{SMIP:obj} minimizes the summation of the core slice provisioning cost and the expectation of the second stage objective which is the RAN slice provisioning cost. $\eta$ is a constant parameter that determines the balance between the objectives of the first and second stages.
% The constraint sets \eqref{node_cap1} and \eqref{link_cap1} ensure that the demand allocated to each substrate core node and fronthaul link does not exceed its capacity. The constraint set \eqref{link_cap2} ensures that the demand allocated to each substrate backhaul link does not exceed its capacity. Constraint \eqref{placement1} guarantees that each core VNF is placed at one core substrate node. Finally, the domain constraints are expressed in \eqref{domain1}.The second stage problem objective in \eqref{obj2} minimizes the BW consumption. Constraint \eqref{path2} and  \eqref{path1} enforce the existence of a path in the substrate network for each virtual backhaul and fronthaul link. Constraint \eqref{rate} guarantees that the rate of gNB $v$ allocated to slice $k$ to be greater than the total demand of the users covered by $v$. Constraint \eqref{cap_ran} limits the load allocated to a gNB to the maximum traffic that can be supported by the gNB. Constraint \eqref{placement2} ensures that a virtual gNB of slice $k$ is placed at a gNB if at least one user of that slice is covered by that gNB. The domain constraints for the second-stage problem is expressed by \eqref{domain2}.



==> formulation2.tex <==
\section{System Model and Problem Formulation}
We consider the resource provisioning problem of mobile network slicing across both RAN and core components. In this section, the network and slice models are presented followed by problem formulation.
\label{sec:sys}
% We consider the The 5G NS resource allocation problem has two domains, the radio and the core (transport) network resource allocations. While these two problems can be solved separately, a joint approach is more sensible considering the uncertainty about demand points locations. However, obtaining the optimal decision which minimizes the overall cost is not trivial in this case. We propose a two-stage stochastic optimization framework to tackle this problem. In the following, the network and slice models are presented and then the proposed problem formulation is detailed.
\subsection{Infrastructure Network model}
Let the infrastructure network (substrate) be represented as a directed graph $G = (V, E)$, where $V$ is the set of infrastructure nodes and $E$ denotes the set of infrastructure links. The set of infrastructure network nodes consist of two type of nodes, gNB and non-gNB. Thus, $V = V_{gNB} \cup V_{-gNB}$ where $V_{gNB}$ and $V_{-gNB}$ correspond to the set of substrate gNB and non-gNB node, respectively. Each gNB is characterized by its maximum supported traffic which is computed based on its available bandwidth (physical resource blocks or PRBs) and MIMO antenna configuration. Non-gNBs are general-purpose servers providing essential capabilities for running core network network functions (NFs) and could data centers. A substrate node is characterized by its available CPU, storage and RAM resources. We define the set of node resources as $\mathcal{T} = \{CPU, STO, RAM\}$. Let the vector $W_j = (W^{CPU}_j, W^{STO}_j, W^{RAM}_j)$ represent the available capacity of the substrate node $j$. These amounts correspond to the initial capacity of the node reduced by the amount allocated to previously accepted concurrent requests. Moreover, the cost of each infrastructure node $j$ being used by a VNF consist of two parts: (i) a fixed part $C_j$ paid for each VNF deployed on node $j$, (ii) a variable part associated to the per-unit usage of each resource which depends linearly on the amount of the resource consumed by a VNF. The per-unit variable cost corresponding to CPU, storage and memory of node $j$ are denoted by $C_j^{CPU}, C_j^{STO} $ and $C_j^{RAM}$. 

We assume that the available
spectrum of gNB $j\in V_{gNB}$ is divided into a set of $W^{RAN}_j$ physical resource blocks (PRBs)  can be allocate to different users of different slices \cite{} \cite{papa2021user}. Furthermore, the set of infrastructure link $E = E_{FH} \cup E_{BH}$ where $E_{FH}$ and $E_{BH}$ stand for the links between gNB nodes and the core network and the remaining link, respectively. Each substrate link $e\in E$ has a bandwidth capacity and propagation delay denoted by $W^{BW}_e$ and $\tau^{PRO}_e$ in respective order. Moreover, a per-unit bandwidth cost is associated to the infrastructure link $e$ denoted by $C_e^{BW}$. In order to meet the traffic transmission between two VNFs of a network slice, we consider a set of substrate paths denoted by $\mathcal{P}$. Let $\mathcal{P}( i \rightarrow j )$ denote the set of substrate path between $i$ and $j$. Therefore, $\mathcal{P} = \cup_{i,j\in V, i\neq j} \mathcal{P}( i \rightarrow j )$.
% For the sake of simplicity, we assume that each UE is covered by one gNB and gNBs do not interfere. 

We consider an environment in which MUs submit their request for different services to SPs. For the sake of simplicity, we assume that each user requests at most one service. This can be readily extended to the case with multiple requests from a user by duplicating MUs which have multiple service requests. Each service is realized through network slices managed by SPs. The SPs meet their customers requested services by dedicating network slices with specified QoS requirements deployed on the substrate network which is owned and managed by InPs. Let $U$ denoted the set of MUs distributed across the considered geographical area. We assume that each MU is served by a gNB according to the nearest association rule. 

For a user 
%and $\mathcal{K}$ and the set of network slices
% Therefore, the set of MUs served by gNB $v\in V_{gNB}$ and requesting the service met by slice $k\in \mathcal{K}$ is represented by $U_v^k$.


\subsection{Network Slice Model}
In this section, we present the network slice model. We assume that a slice request is modeled as one or multiple service function chains (SFCs), each consisting of a number of VNFs (e.g. gNB , AFM, UPF, SMF) and virtual links (VLs) between them. The set of system network slices is represented by $\mathcal{K}=\{1,...,K\}$. Let the directed graph $G^\prime_{k} = (V^\prime_{k}, E^\prime_{k})$ describe the $k$th slice' SFCs. Similarly to the substrate network, we assume that the nodes of slice $k$ consists of two types of nodes, gNB and non-gNB. Therefore, $V^\prime_{k} = V^\prime_{k,gNB} \cup V^\prime_{k,-gNB}$ where $V^\prime_{k,gNB}$ and $V^\prime_{k,-gNB}$ correspond to the set of gNBs and non-gNB functions of slice $k$. Moreover, $E^\prime_{k} =  E^\prime_{k, FH}\cup E^\prime_{k, BH}$ where $E^\prime_{k, FH}$ and $E^\prime_{k, BH}$ denote the fronthaul and backhaul VLs, respectively. 
We assume that each instance of the SFC corresponding to slice $k$ has QoS requirements expressed as gNB's radio resource $r_k$ and maximum E2E tolerable latency $d_k$. In addition, each VNF instance of the node $j^\prime$ in slice $k$ requires the CPU, storage and RAM resources, represented by the vector $R_{j^\prime}= (R^{CPU}_{j^\prime}, R^{STO}_{j^\prime}, R^{RAM}_{j^\prime})$. Similarly, each VL $e^\prime \in E^\prime_{k}$ is characterized by the bandwidth requirement of $R^{BW}_{e^\prime}$ to meet the demand for data transmission between the two end-pints (VNFs) of $e^\prime$. We assume that the traffic flow of each $e^\prime \in E^\prime_k$ is routed through substrate paths. Therefore, we represent the set of substrate paths considered for slice $k$ edges by $\mathcal{P}_k$, where $\mathcal{P}_k \subseteq \mathcal{P}$.

In order to satisfy the demands of all users requesting a network slice, multiple instances of that slice may be required to be deployed. We define the parameter $u_v^{k,i}$ which is equal to $1$ if user $i$ of slice $k$ is covered by gNB $v$ and $0$ otherwise. Moreover, the parameter $I_k$ indicates the number of instances of slice $k$ needed to be deployed in order to support the demand for slice $k$. Due to the mobility of the MUs and their varying demands, the true values of $u_v^{k,i}$ and $I_k$ are not known. However, given the historical data on the demand and mobility patterns of MUs, the SP and InP are capable of estimating the statistical characteristics of $u_v^{k,i}$ and $I_k$. 
%**** In order to speed up the reconfiguration process and minimize VNF migrations resulted from users mobility and change of covering gNB, we assume that all instances of the core VNFs for a NS are embedded on one substrate node in contrast to the virtual gNBs that are essentially placed on different substrate gNBs as required. 
\begin{figure}[!t]
\centering
\includegraphics[width=0.30\textwidth]{figures/slice_example.png}
  \caption{A network slice example}
    \label{fig:slice}
\end{figure}
\begin{table*}[t]
\centering
\begin{center}
\scalebox{1}{
\begin{tabular}{c|c}
\hline
\hline
Network Parameters & Description\\
\hline
$G = (V, E)$ & Substrate network graph\\
$V_{gNB}, V_{core}$ & Set of substrate gNB and non-gNB nodes\\
% $E_{FH}, E_{BH}$ & The set of fronthaul and backhaul links\\
$\mathcal{P}$ & Set of Substrate paths\\
$W_{v}^{tr}$ & Available spectrum of gNB $v$\\
$U^k$ & Number of users of slice $k$ in the network\\
$W_j^{CPU,STO,RAM}$ & The amount of CPU, Storage and RAM capacities of the substrate node $j$\\
$W_e^{CAP}$ & The capacity of the substrate link $e$\\
\hline
\hline
Slice Parameters & Description\\
\hline
$K$ & Number of requested slices\\
$G^k_{slc} = (V_{slc}^k, E_{slc}^k)$& The $k$th slice SFC graph\\
$V^k_{slc,ran}, V^k_{slc,core}$ & the set of virtual RAN and core VNFs\\
$E_{slc, FH}^k, E_{slc, BH}^k$ & The set of fronthaul and backhaul virtual links\\
$r_k$ & slice $k$ rate requirement\\
$R_{j^\prime}^{CPU, STO, RAM}$ & The amount of CPU, Storage and RAM resource requirements of the VNF $j^{\prime}$\\
$R_{e^\prime}^{CAP}$ & The data rate requirement of the virtual link $e^\prime$\\
\hline
\hline
\end{tabular}}
\end{center}
\caption{System model parameters}
\label{parameters}
\end{table*}

\begin{itemize}
\item $I_k$: number of virtual gNBs supported by slice $k$ core (not a random variable)
\item $\chi_k$: scaling factor of BW, compute and storage resources for slice $k$
\end{itemize}
\subsection{Two-timescale resource reservation framework}
%change the sentences! is directly form another paper
We assume the lifecycle of resource management for the considered network slices is set to be one day. The reason that we choose the resource management lifecycle of a slice as one
day is because this lifecycle exhibits the property of periodicity.
The user traffic may vary during different time of the day. The
variation of user traffic may follow a certain pattern during the
day. We divide 24 hours into $Q$ long timescale slots (minutes). We assume that at long time slot $q$, the spatial distribution of demand points for $K$ different network slices are given, represented by $\mathcal{F}_1,\dots,\mathcal{F}_k, k\in \mathcal{K}$. Hence, $u_v^{k,i}$ and $I_k$ become random variables with known distributions. Define $\mathcal{F}^q = \{\mathcal{F}_1^q,\dots,\mathcal{F}_k^q\}, k\in \mathcal{K}$.
Each long timescale slot consists of $T$ short timescale slots
with the same duration. Resource reservation for the considered
slice is updated at the beginning of each long timescale slot
with the statistical knowledge of user traffic. Intra-slice resource
allocation is performed over short timescale under an arbitrary
user arrival/departure process. The choice of the duration of each
long timescale slot should guarantee that the statistics of user
\subsection{Problem formulation}
% Figure \ref{fig:architecture} illustrates an example of E2E resource allocation for different slices. 
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/architecture.png}
%   \caption{An example of the E2E slice resource allocation}
%     \label{fig:architecture}
% \end{figure} 
% The problem architecture is illustrated at the bottom of this figure.
%The main consideration is that the problem is solved for a set of gNBs connected to a single gateway acting as an aggregation point. 
Given the substrate network and network slice graphs, we formulate the problem of E2E network slicing under demand uncertainty as a two-stage SMIP, using the following variables:
\begin{itemize}
\item A set of binary variables $\boldsymbol{x}_{k}$ where $x_j^{k,j^\prime}$ is $1$ if the an instance of VNF $j^\prime$ of the $k$th slice is placed at substrate node $j$.
\item A set of binary variables $\boldsymbol{y}_{k}$ where $y_p^{k,e^\prime}$ is 1 if the virtual link $e^\prime$ of the $k$th slice is assigned to substrate path $p$.
\item A set of continuous decision variables $\boldsymbol{z}_k$ where $z_j^k$ represents the fraction of gNB $j$ supported traffic that is allocated to slice $k$.
\end{itemize}
It is important to note that the value of the vector $\boldsymbol{z} = (z_1^1,...,z_{|V_{gNB}|}^1,...,z_1^K,...,z_{|V_{gNB}|}^K)$ represents the RAN slicing policy defined as the fraction of each cell available radio resource that is assigned to each requested slice. For example, in the case of having three network slices, the resulted RAN slice allocation for an gNB can be $20\%, 50\% $ and $30\%$. Once this spectrum assignment policy is determined, the actual radio resource allocation in terms of the number of PRBs allocated to the users of each slice to fulfill the spectrum requirement is formulated separately. In this regard, different solutions have been proposed in the literature with the goal of minimizing the interference between different mobile virtual network operators \cite{RAN}. 

We model the resource provisioning problem for the requested slices as a two-stage SMIP. We refer to this method as \textbf{SMIP} which is described in the following sections.

\subsubsection{First-stage problem}
The first-stage objective in \textbf{SMIP} is the minimization of the total provisioning cost which consists of node and link deployment costs for all slices. Let $\mathcal{C}_k^{N}$ and $\mathcal{C}_k^{L}$ denote the node and link costs corresponding to slice $k$, respectively. Consequently, we have:
% \begin{strip}
\begin{equation}
    \mathcal{C}_k^N(\boldsymbol{x}_{k}) = \sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}C_j^kx_{j}^{k}+\sum_{j\in V} \sum_{j^{\prime}\in V^\prime_{k}}\sum_{t\in \mathcal{T}}R_{j^\prime}^tC_j^t x_j^{k,j^\prime}
    \label{SMIP:node-cost}
\end{equation}
\begin{equation}
    \mathcal{C}_k^L(\boldsymbol{y}_{k}) = \sum_{p\in\mathcal{P}}\sum_{e\in p}\sum_{e^\prime \in E^\prime_k} R_{e^\prime}^{BW} C_e^k y_{p}^{k, e^\prime}
    \label{SMIP:link-cost}
\end{equation}
% +\phi_2\sum_{e\in E}\sum{e^\prime \in E^\prime_k} z_{e}^{k, e^\prime} C_e^k) +\phi_3\mathbb{E} Q_{x,z}(u)
where
\begin{equation}
  x_{j}^{k} =
    \begin{cases}
      1 & \text{if $\sum_{j^\prime\in V^\prime_{k}}x_j^{k,j^\prime} \geq 0$}\\
      0 & \text{otherwise}
    \end{cases}       
\end{equation}
Hence, the first-stage objective is: \begin{equation}
     \mathcal{C}_1 (\boldsymbol{x},\boldsymbol{y}) = \phi_1\sum_{k\in\mathcal{K}}\mathcal{C}^N_k(\boldsymbol{x}_k)+\phi_2 \sum_{k\in\mathcal{K}}\mathcal{C}^L_k(\boldsymbol{y}_k)
     \label{SMIP:Obj1}
\end{equation}
where $\phi_1$ and $\phi_2$ are constants to balance between the two objective terms of \eqref{SMIP:node-cost} and \eqref{SMIP:link-cost}.
% +\phi_3\mathbb{E} Q_{x,y}(U)

For each infrastructure node and link, we have capacity constraints as follows:
\begin{equation}
    \text{C1}:\ \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \chi_k \leq W_j^{t} \quad t\in \mathcal{T}, \forall j\in V_{} \label{SIMP:node-Cap1}
\end{equation}
\begin{equation}
    \text{C2}:\ \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} \chi_k \leq W_e^{BW} \quad \forall e \in E
    \label{SIMP:link-Cap1}
\end{equation}
Moreover, in a feasible resource provisioning solution, each gNB VNF is placed at one substrate gNB node and each non-gNB VNF runs on a substrate non-gNB node. Thus, the resulting VNFs deployment must guarantee the following constraints:
% \begin{equation}
%     \text{C3}:\ \sum_{j\in V_{gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,gNB}
%     \label{SIMP:gNB-map1} -->removed
% \end{equation}
\begin{equation}
    \text{C3}:\ \sum_{j\in V_{-gNB}}x_j^{k,j^\prime} = 1 \quad \forall k \in \mathcal{K}, j^\prime \in V^\prime_{k,-gNB}
    \label{SIMP:non-gNB-map1}
\end{equation}
Let $\mathcal{P}^\prime_k$ denote the set all paths of slice $k \in \mathcal{K}$. The execution latency of VNF $j^\prime \in V^\prime_k$ on infrastructure node is represented by $\tau^{k,j^\prime}$. Given the edge mapping decision variables $y^{k,e^\prime}_p$, the data transmission latency corresponding to the infrastructure edge $e\in E$ based on its aggregated assigned data demand is computed in equation \eqref{d-edge}.
\begin{equation}
    \sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e} \label{d-edge}
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ mapped to the path $p\in \mathcal{P}_k$ is:
\begin{equation}
    \sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]
\end{equation}
Thus, the latency of the VL $e^\prime \in E^\prime_k$ is computed in equation \eqref{d-slice-edge}.
\begin{equation}
    \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \label{d-slice-edge}
\end{equation}
The latency of slice $k$ instances experienced by the MUs of that slice is guaranteed to be lower than the required latency of the slice in constraints \eqref{SIMP:latency-1}.
\begin{align}
    & \text{C4}: \nonumber\\
    & \sum_{e^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{p\in\mathcal{P}_k} y^{k,e^\prime}_p \left[\sum_{e\in p} \left[\sum_{k\in\mathcal{K}} \sum_{p\in\mathcal{P}_k:e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p \frac{R^{BW}_{e^\prime}}{W^{BW}_e}\right]\right] \right]\nonumber\\
    & + \sum_{j^\prime \in \mathcal{P}^\prime_k} \left[ \sum_{j\in V} x^{k,j^\prime}_j \tau^{k,j^\prime} \right]  \leq d_k\quad \forall p^\prime \in \mathcal{P}^{\prime}_k, k\in \mathcal{K} \label{SIMP:latency-1}
\end{align}
Finally, the domain constraints are presented as follows:
\begin{align}
    & \text{C5}: 
    x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \ k\in \mathcal{K}, j\in V, j^\prime \in V^\prime_k, p\in \mathcal{P}_k, e^\prime \in E^\prime_k \label{SMIP:dom1}
\end{align}
% \begin{align}
%&\textbf{s.t} \nonumber \\
%& \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% &\sum_{e\in\delta^+(j)} z_{e}^{k, e^\prime} - \sum_{e\in\delta^-(j)}z_{e}^{k, e^\prime} = 
    %\left\{
    %\begin{array}{@{}ll@{}}
    %1 & if \quad j = destination(e^\prime)\\
    %-1 &  if \quad j = source(e^\prime)\\
    %0 & otherwise\\
    %\end{array}\right. \quad k=1,...,K, \forall j \in V, e^\prime \in E^k_{slc} \label{path}\\
% &\sum_{k=1}^K \sum_{j^\prime\in V_{slc}^k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \leq W_j^{t} \quad t\in \{CPU, STO, RAM\}, \forall j\in V_{} \label{node_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,FH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{FH}\label{link_cap1}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc,BH}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{BH}\label{link_cap2}\\
% &\sum_{k=1}^K \sum_{e^\prime \in E^k_{slc}}z_{e}^{k,e^\prime} R_{e^\prime}^{CAP} \leq W_e^{CAP} \quad \forall e \in E_{}\label{link_cap1}\\
% &\sum_{j\in V_{core}}x_{j}^{k,j^\prime} = 1 \quad k=1,...,K, \forall j^\prime \in V^k_{slc,core} \label{placement1}\\
% & x_j^{k, j^\prime}\in \{0,1\}, z_{e}^{k,e^\prime} \geq 0  \quad k = 1,...,K, j\in V, j^{\prime}\in V^{k}_{slc}, e\in E, e^\prime \in E^k_{slc} \label{domain1}
% \end{align} 
% \end{strip}
The flow conservation constraints are guaranteed by equations \eqref{SIMP:flow2-nongNB} and \eqref{SIMP:flow2-gNB}.  
\begin{align}
    & \text{C6}:\ \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime} \nonumber\\
    &\qquad\qquad\forall k\in\mathcal{K},  e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{SIMP:flow2-nongNB}
\end{align}
\begin{align}
    & \text{C7}:\ \sum_{\substack{p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\  j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} - y_{q(j \rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_{k} \nonumber \\
    &\qquad\qquad \forall k\in \mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime \rightarrow j^\prime)\in E_{k,FH}^\prime \label{SIMP:flow2-gNB}
\end{align}

%%second stage
\subsubsection{Second-stage problem} The goal of the second-stage problem is to minimize the total gNB traffic allocated to network slices. 
The second-stage objective is:
\begin{equation}
     \mathcal{C}_2(\boldsymbol{z}) = \sum_{k\in\mathcal{K}}\sum_{j\in V_{gNB}} z^k_{j}
\end{equation}
% \begin{align}
%     & \text{C8}:\ c k_i (1-BER_i) \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\
%     &\quad \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
% \end{align}
The traffic allocated to the users of a slice must be greater than the required traffic of slice k. This constraint is ensured by equations \eqref{SIMP:reqrate}.
\begin{align}
    & \text{C8}:\ z_j^k W_j^{RAN} \geq x^{k,j^\prime}_j\sum_{i = 1}^{U_k} r_k u_{i,j}^k \nonumber \\ 
    & \forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:reqrate}
\end{align}
\begin{align}
    & \text{C8:} \frac{\sum_{i=1}^{U_k}u^k_{i,j}}{\sum_{k=1}^K\sum_{i=1}^{U_k}u^k_{i,j}} \leq z^k_j\ \forall j\in V_{gNB} \label{SIMP:reqrate}
\end{align}
The capacity constraint of gNBs is enforced by equation \eqref{SIMP:gNBcap}. 
% \begin{equation}
%     \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq W_j^{tr} \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
% \end{equation}
\begin{equation}
    % \text{C9}:\ \sum_{k=1}^K \sum_{i=1}^{U_k} z_{i,j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
    \text{C9}:\ \sum_{k=1}^K z_{j}^k \leq 1 \quad \forall j\in V_{gNB} \label{SIMP:gNBcap}\\
\end{equation}
The gNB placement constraints are enforced by equation \eqref{SIMP:gNBplacement2}.
\begin{equation}
    \text{C10}: \ x_j^{k, j^\prime} = \mathbbm{1}_{\{\sum_{i=1}^{U_k} u_{i,j}^k\geq1\}} \forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime \label{SIMP:gNBplacement2}\\
\end{equation}
The domain constraints of the second-stage problem are:
\begin{align}
    & \text{C11}: \ z^k_j \in [0, 1] \quad \forall k\in \mathcal{K}, j\in V_{gNB},  \label{domain2} 
\end{align}
% Let $Q(\boldsymbol{x},\boldsymbol{y}, U)$ denote the optimal value of the second-stage problem. 
The E2E network slicing problem with demand uncertainties is formulated as a two-stage SMIP presented below:
\begin{align}
    & {minimize} \quad \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) + \eta \ \mathbb{E}_{
    \mathcal{F}} [min \ \mathcal{C}_2 (\boldsymbol{z})] \label{SMIP:obj} \\
    & \qquad \qquad \qquad \text{s.t.}  \qquad \text{C1}-\text{C11} \nonumber
\end{align}
% $Q_{x,z}(u)$ is the optimal value of the second-stage defined as follows:
% \begin{strip}
% \begin{align}
% &\textbf{minimize}
% \quad \sum_{k=1}^{K} (\sum_{v\in V_{gNB}} z_k^v) \label{obj2}\\
% &\textbf{s.t} \nonumber \\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{j}^{k,m}-x_{j}^{k,n})I_{k} \quad k = 1,...,K, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path2}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path1}\\
% & y_k^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{U_k} r_k u_{k,i}^v \quad k =1,...,K, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate}\\
% &\sum_{k=1}^K y_k^v \leq W_v^{tr} \quad \forall v\in V_{gNB} \label{cap_ran}\\
%&\sum_{}z_{e}^{e^\prime , k}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{U_k} u_{i,k}^j\geq1\}} \quad k = 1..., K, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement2}\\
% & y_k^v \in [0, W_v^{tr}], \quad k = 1..., K, \forall  v\in V_{gNB},  \label{domain2}
% \end{align}
% \end{strip}
The objective \eqref{SMIP:obj} minimizes the summation of the core slice provisioning cost and the expectation of the second stage objective which is the RAN slice provisioning cost. $\eta$ is a constant parameter which determines the balance between the objectives of the first and second stages.
% The constraint sets \eqref{node_cap1} and \eqref{link_cap1} ensure that the demand allocated to each substrate core node and fronthaul link does not exceed its capacity. The constraint set \eqref{link_cap2} ensures that the demand allocated to each substrate backhaul link does not exceed its capacity. Constraint \eqref{placement1} guarantees that each core VNF is placed at one core substrate node. Finally, the domain constraints are expressed in \eqref{domain1}.The second stage problem objective in \eqref{obj2} minimizes the BW consumption. Constraint \eqref{path2} and  \eqref{path1} enforce the existence of a path in the substrate network for each virtual backhaul and fronthaul link. Constraint \eqref{rate} guarantees that the rate of gNB $v$ allocated to slice $k$ to be greater than the total demand of the users covered by $v$. Constraint \eqref{cap_ran} limits the load allocated to a gNB to the maximum traffic that can be supported by the gNB. Constraint \eqref{placement2} ensures that a virtual gNB of slice $k$ is placed at a gNB if at least one user of that slice is covered by that gNB. The domain constraints for the second-stage problem is expressed by \eqref{domain2}.



==> prelim.tex <==
\section{Stochastic Programming}
\label{sec:prelim}
In this section, we provide a brief overview of stochastic programming \cite{book}. \textit{Stochastic linear programs} (SLP) are linear programs where some data are uncertain, represented as random variables with given probability measures. The values of these random variables are only known after a random experiment. SLP's optimization decision variables are divided into two groups: first-stage variables, determined before the experiment, and second-stage variables, determined after the experiment results are known.
% The value of the random variables are known only after a random experiment. Hence, the set of optimization decision variables in SLP are divided into two groups: (i) first-stage decision variables, (ii) second-stage decision variables. While the first-stage variables are determined before the random experiment, the second-stage decisions are taken after the random experiment becomes known. 
Let $\boldsymbol{x} \in \mathbb{R}^{n_1\times 1}$ denote the vector of first-stage optimization variables. Define the random variable corresponding to the unknown data as $\boldsymbol{\xi}=\boldsymbol{\xi}(\omega)$ with $\omega\in \Omega$ representing a random event. The vector of second-stage decision variables is denoted by $\boldsymbol{y}(\omega,\boldsymbol{x})$. We assume that the probability distribution $\mathcal{F}$ on $\Omega$ is known in the first stage. The classical two-stage SLP with \textit{fixed recourse} is formulated as follows:
\begin{align}
    & minimize \quad \boldsymbol{c}^T \boldsymbol{x} + \mathbb{E}_{\mathcal{F}}[min\ \boldsymbol{q}(\omega)^T \boldsymbol{y}(\omega,\boldsymbol{x})] \label{SLP-obj}\\
    & s.t. \quad A\boldsymbol{x} = \boldsymbol{b}\label{SLP-c1}\\
    & T(\omega)\boldsymbol{x} + W \boldsymbol{y}(\omega,\boldsymbol{x}) = \boldsymbol{h}(\omega)\label{SLP-c2}\\
    & \boldsymbol{x},\boldsymbol{y}(\omega,\boldsymbol{x}) \geq \boldsymbol{0} \label{SLP-c3}.
\end{align}
where $\boldsymbol{c}\in \mathbb{R}^{n_1\time 1}, \boldsymbol{b}\in \mathbb{R}^{m_1\times 1}, A\in \mathbb{R}^{m_1\times n_1}$. The objective function \eqref{SLP-obj} consists of the deterministic term $\boldsymbol{c}^T \boldsymbol{x}$ and the expectation of the term $\boldsymbol{q}(\omega)^T \boldsymbol{y}(\omega,\boldsymbol{x})$ over all realizations of the random event $\omega$. Note that once the random event $\omega$ is realized, $T(\omega) \in \mathbb{R}^{m_2\times n_2}, \boldsymbol{h}(\omega) \in \mathbb{R}^{m_2\times 1}$, and $\boldsymbol{q}(\omega)\in \mathbb{R}^{n_2\times 1}$ become known. In particular $\boldsymbol{\xi}(\omega) = (\boldsymbol{q}(\omega), \boldsymbol{h}(\omega), T_1(\omega),\dots,T_{m_2}(\omega))$ represents the random data vector where $T_1(\omega),\dots,T_{m_2}(\omega)$ are the rows of $T(\omega)$. For a given $\omega$, let $Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))$ denote the value of the second-stage problem, defined as:
\begin{align}
    & Q(\boldsymbol{x},\boldsymbol{\xi}(\omega)) = min_{\boldsymbol{y}\geq 0} \{\boldsymbol{q}(\omega)^T \boldsymbol{y} | W\boldsymbol{y} = \boldsymbol{h}(\omega)-T(\omega)\boldsymbol{x}\} \label{2-stage-value}
\end{align}
Moreover, the expected value of the second-stage objective value is defined as:
\begin{align}
    & \mathcal{Q}(\boldsymbol{x}) = \mathbb{E}_{\mathcal{F}}[Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))] \label{2-stage-expected-value}
\end{align}
Then, the \textit{deterministic equivalent program} (DEP) corresponding to \eqref{SLP-obj}-\eqref{SLP-c3} is defined as:
\begin{align}
    & min \quad \boldsymbol{c}^T \boldsymbol{x} + \mathcal{Q}(\boldsymbol{x}) \label{DEP-obj}\\
    & s.t. \quad A\boldsymbol{x} = \boldsymbol{b} \label{DEP-c1}\\
    & \boldsymbol{x} \geq \boldsymbol{0} \label{DEP-c2}
\end{align}
The DEP formulation illustrates the major difference between a deterministic linear program and a SLP. Given $\mathcal{Q}(\boldsymbol{x})$, a SLP is an ordinary nonlinear program due to the nonlinearity of $\mathcal{Q}(\boldsymbol{x})$. On the other hand, the computation of $\mathcal{Q}(\boldsymbol{x})$ requires the evaluation of $Q(\boldsymbol{x},\boldsymbol{\xi}(\omega))$ for all $\boldsymbol{x}$ and $\omega$ which is not possible in practice. The problem becomes even more challenging considering the first-stage or second-stage variables to be integers, e.g. $\boldsymbol{x}\in \mathbb{Z}^{n_1}_+$, $\boldsymbol{y}\in \mathbb{Z}^{n_2}_+$. In the next section, we first present our system model for the \emph{network slicing} problem with demand uncertainties followed by our proposed formulation which is based on two-stage stochastic mixed-integer programming. 

==> solution.tex <==
\section{Proposed Solution}
\label{sec:solution}
\subsection{Deterministic Equivalent Reformulation and Sample Average Approximation (SAA)}
In this section, we introduce the deterministic reformulation of the modeled \textbf{SMIP} and then propose a solution based on the sample average approximation (SAA). The SAA method is an approach for solving stochastic optimization problems by using Monte Carlo simulation. Suppose that $H$ realization of the random variables $\chi_k$ and $u_{i,j}^k$, $U_k$ are available denoted by $\hat{\chi}_{k,h}$, $\hat{u}_{i,j,h}^k$,$\hat{U}_{k,h}$, $h = 1,...,H$. For each realization, we have a separate second-stage variable $z_{j,h}^k$. We convert \textbf{SMIP} to its sampled deterministic equivalent problem, defined as follows:
% \begin{strip}
\begin{align}
% \begin{gather*}
% &{minimize} \quad \medmath{\sum_{k=1}^{K} \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) +\phi_3 \sum_{h=1}^H p_h \mathcal{C}_2(\boldsymbol{z}_h)}
% \label{obj_det} \\
&{minimize} \quad \mathcal{C}_1(\boldsymbol{x},\boldsymbol{y}) +\eta \sum_{h=1}^H \frac{1}{H} \mathcal{C}_2(\boldsymbol{z}_h)
\label{obj_det} \\
&{s.t.} \qquad \qquad \qquad \text{C3,C4}, \text{C6,C7} \label{constraints-moved}\\
& \text{C12}:\ \sum_{k\in \mathcal{K}} \sum_{j^\prime\in V^\prime_k} x_{j}^{k,j^\prime} R_{j^\prime}^{t} \hat{\chi}_{k,h} \leq W_j^{t} \quad \forall t\in \mathcal{T}, j\in V_{}, h\in\mathcal{H} \label{}\\
& \text{C13}:\ \sum_{k\in\mathcal{K}} \sum_{p\in \mathcal{P}_k: e\in p}\sum_{e^\prime \in E^\prime_k} y^{k,e^\prime}_p R^{BW}_{e^\prime} \hat{\chi}_{k,h} \leq W_e^{BW} \quad \forall e \in E, h\in\mathcal{H} \label{}\\
% & \text{C14}: \sum_{\substack{{}p(i\rightarrow j),q(j\rightarrow i) \in \mathcal{P}\\ j\in V}} y_{p(i\rightarrow j)}^{k,e^\prime} -y_{q(j\rightarrow i)}^{k,e^\prime} = (x_{i}^{k,i^\prime}-x_{i}^{k,j^\prime})I_k \nonumber\\
% &\forall k\in\mathcal{K}, i\in V_{-gNB}, e^\prime(i^\prime\rightarrow j^\prime) \in E^\prime_{k,BH} \label{path1_det}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = (x_{i}^{k,m}-x_{i}^{k,n})\hat{I}_{k,h} \quad k = 1,...,K, h=1,...,H, \forall i\in V_{core} , (m,n)\in E_{slc}^k \label{path1_det}\\
% & \sum_{j\in V} z_{(i,j)}^{k,(m,n)} - z_{(j,i)}^{k,(m,n)} = x_{i}^{k,m}-x_{i}^{k,n} \quad k = 1,...,K, \forall i\in V_{gNB} , (m,n)\in E_{slc,FH}^k \label{path2_det}\\
& \text{C15}: \ z_{j,h}^k W_j^{tr} \geq x^{k,j^\prime}_j\sum_{i = 1}^{\hat{U}_{k,h}} r_k \hat{u}_{i,j,h}^k \nonumber \\ 
&\forall k\in\mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in\mathcal{H} \label{rate_det}\\
% & y_{k,h}^v \geq x^{k,j^\prime}_v\sum_{i = 1}^{\hat{U}_{k,h}} r_k \hat{u}_{k,i,h}^v \quad k =1,...,K, h=1,...,H, \forall v\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{rate_det}\\
& \text{C16}: \ \sum_{k=1}^K z_{j,h}^k \leq 1 \quad \forall j\in V_{gNB}, h\in\mathcal{H} \label{cap_ran_det}\\
% &\sum_{k=1}^K y_{k,h}^v \leq W_v^{tr} \quad h=1,...,H, \forall v\in V_{gNB} \label{cap_ran_det}\\
& \text{C17}: \ x_j^{k, j^\prime} = \mathbbm{1}_{\{\sum_{i=1}^{\hat{U}_{k,h}} \hat{u}_{i,j,h}^k\geq1\}}\nonumber\\ &\forall k\in \mathcal{K}, j\in V_{gNB}, j^\prime \in V_{k,gNB}^\prime, h\in\mathcal{H} \label{placement_det2}\\
% & x_j^{k, j^\prime} = \mathbbm{1}{\{\sum_{i=1}^{\hat{U}_{k,h}} \hat{u}_{k,i,h}^j\geq1\}} \quad k = 1..., K, h=1,...,H, \forall j\in V_{gNB}, j^\prime \in V_{slc,ran}^k \label{placement_det2}\\
% & x_j^{k,j^\prime}, y^{k,e^\prime}_p \in \{0,1\} \quad \forall j\in V, j^\prime \in V^\prime_k, p\in\mathcal{P}_k, e\in E^\prime_k, k\in \mathcal{K}\nonumber \\
& \text{C18}: \quad z^k_{j,h} \in [0,1] \ \forall k\in \mathcal{K}, j\in V_{gNB}, h=1,\dots,H \label{domain_det}
% \end{gather*}
\end{align}
% \end{strip}
We refer to the above problem as \textbf{DET}\_\textbf{MILP}. The first term in the objective function \eqref{obj_det} is same as the first term of the objective function \eqref{SMIP:obj}. The second term is the weighted average of the the second stage objective function over the $H$ realized samples of the random variables $I_k, u^k_{i,j}$ and $U_k$. Constraints C12, C13, C14, C15, C16 replace their counterparts C6, C8, C9, C10, C11 respectively.

In the evaluation section, the performance of this methods is benchmarked against the strategy of providing resources for the worst case scenario, which is the aligned with the way many networks are managed in reality.
%disadvantages: large scale problem, The disadvantage of sampling approaches: some efforts might be wasted on optimizing when distribution approximation is not accurate \cite{book}. 
%Two ways to reduce the problem: Importance sampling and stochastic decomposition.
% \subsection{L-shaped method with implicit enumeration}
% In order to alleviate the complexity arising from large scale second-stage variables and the binary first stage variables, we exploit an integer L-shaped method in this section based on \cite{wo}. 

% \subsection{Adaptive RAN slicing} 

